ProsaBuddy: Assisting Mechanized Real-Time Schedulability Analysis with LLM-based Agents

Rigorous schedulability analysis is essential for the design of hard real-time systems, yet errors in pen-and-paper proofs threaten the safety of critical applications. The Prosa initiative addresses this by offering a foundation for building machine-checkable schedulability analysis proofs in the Rocq proof assistant. However, the substantial time and expertise required to construct such proofs remain a major barrier for wider adoption of Prosa. This work presents ProsaBuddy, an LLM?based agent system designed to lower the effort needed to develop mechanized real-time schedulability proofs. ProsaBuddy employs a ReAct loop with retrieval over the Prosa codebase, access to Rocq tools and optional human-written hints. It uses a subgoal?delegation architecture, decomposing a lemma into subgoals and dispatches them to subagents for proof. We evaluate ProsaBuddy on a mini benchmark drawn from real-time scheduling literature. Experiment results show that ProsaBuddy significantly outper?forms state-of-the-art LLM-based Rocq automated proving agent systems and a general coding agent OpenCode

==> sections/acknowledgment.tex <==
\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.


==> sections/appendex.tex <==
\section{Appendix}



==> sections/background.tex <==

\guan{introduce the structure of Rocq statement: what is formalization, Variable, Definition, Hypothesis, Context, Lemma, goal, tactics, admit, ... }

\guan{
\begin{itemize}
    \item context keyword is a special way to define variables
    \item 
\end{itemize}
}


\guan{to unify the terminology, lemma, theorem, goal, subgoal}

\guan{goal}

\guan{have}

\guan{proof obligation}

\guan{coqc engine, coq tools, we define a term called coq tools as the general name, then each individual name}
\ljy{ All Use Rocq , write something to claim    }


\guan{introduce the Rocq tools}

Coq/Rocq is an interactive theorem prover based on the Calculus of Inductive Constructions (CIC) \cite{??}, a dependent type theory. In CIC, there is no fundamental separation between terms, types, and propositions: logical statements are encoded as types, and a proof of a statement is a program (a term) that inhabits that type. This \enquote{propositions-as-types, proofs-as-programs} paradigm means that specifying a lemma and proving it are both done in the same functional programming language Gallina \cite{??}.
In Coq/Rocq, the usual logical symbols are not built-in primitives but are defined via inductive types. 



To formalize a lemma in Coq/Rocq, it includes the following contents:

\begin{itemize}
  \item \textbf{\texttt{Definition}} -- introduces a computable constant or function with an explicit 
  body. Definitions are \emph{transparent}: they unfold during computation and proof reduction.

  \item {\texttt{Variable}} -- declares a named object without providing its implementation. Variables represent assumptions or undefined parameters of the system. They have no computational content. 

  \item {\texttt{Hypothesis}} -- states an assumption about the variables. Hypotheses form the context from which a lemma must derive its conclusion.

 \item \texttt{Lemma} --  declares a statement to be proved, followed by a proof script. A lemma has a type (the proposition) and a proof term (the evidence). Unlike \texttt{Definition}, which computes a value, a lemma establishes a logical fact. 
\end{itemize}

\guan{introduce admit, goal}

\begin{figure}   
  \centering          
  {
      \includegraphics[width=0.48
      \textwidth]{Coq_basecase.png}
  }
  \caption{An example of a scheduling case in Rocq} 
        
\end{figure}

\guan{Figure \ref{??} shows an example of a lemma.}




\guan{Figure \ref{??}} shows an example of a lemma and its proofs in Coq/Rocq.

To prove a statement, one writes:

\ljy{
Coq basic
\begin{itemize}
    \item Coq/Rocq is an interactive theorem prover that allows users to state mathematical definitions, formulate theorems, and construct machine-checkable proofs. Rocq is the renamed and continuing development of the Coq proof assistant, rather than a fundamentally different prover. The two share the same underlying proof-assistant tradition, logical foundation, and proof-development workflow, but they may differ in naming, versioning, tooling, and some compatibility details across releases. The early versions of PROSA were developed in Coq, while recent versions have migrated to Rocq after this renaming. In this paper, we use the term Coq/Rocq when referring to concepts that are common to both versions, and use Coq or Rocq specifically when discussing version-dependent implementation details. (In the Introduction, we explain that Prosa is built on Coq/Rocq. In the Experiments section, we mention that PROSA 0.4 is based on Coq and PROSA 0.6 is based on Rocq.)
    \item A Coq/Rocq lemma usually consists of more than the final theorem statement. It is stated in a surrounding environment that may include variables, contextual declarations, definitions, hypotheses, and finally the proposition to be proved. The Context command is commonly used to organize variables, assumptions, and typeclass-style parameters that remain available throughout a section or proof.
    \item During an interactive proof, Coq/Rocq maintains a proof state. The proof state records the current goal together with the local hypotheses and definitions that may be used to prove it. Each tactic transforms the proof state: it may simplify the goal, introduce new hypotheses, split the goal into multiple subgoals, or close the current goal completely.
    \item In this paper, we use Lemma and Theorem to refer to top-level propositions that must be proved in Coq/Rocq. A goal is the current proposition that remains to be proved in the proof state. A subgoal is a smaller proof obligation generated either by applying tactics or by explicitly decomposing a larger proof task into smaller parts.
    \item A tactic is a proof command that tells Coq/Rocq how to transform the current proof state. A proof script is a sequence of tactics that eventually closes all generated goals. Common tactics include move for introducing or rearranging hypotheses, rewrite for replacing terms using equalities, apply for using an existing lemma, have, assert, and suff for introducing intermediate facts, case and destruct for case analysis, and lia for solving linear arithmetic goals.
    \item The command admit temporarily skips a local proof obligation, while Admitted accepts an entire theorem without a completed proof. In our system, a proof region refers to a local proof hole that is intentionally isolated and assigned to a subagent for completion. These holes are useful during proof decomposition, but a final verified proof must not contain any remaining admit or Admitted.
    \item Several external tools are useful for interacting with Coq/Rocq proofs. coqc is the compiler that checks whether a .v file is accepted by the prover. coqtop provides an interactive command-line interface for queries such as Check, Search, and Print. coqlsp provides language-server support, including live proof goals, diagnostics, and semantic queries, which are especially useful for iterative proof construction and repair.
    \item In Coq/Rocq, every expression is a formal term, and every term has a type.
A type specifies what kind of object a term is.
For example, \texttt{3} has type \texttt{nat}, \texttt{true} has type \texttt{bool}, and a function such as \texttt{fun x => x + 1} has type \texttt{nat -> nat}.
Propositions are also treated as types: a logical statement is a type, and a proof of that statement is a term inhabiting that type.
Based on this propositions-as-types principle, Coq/Rocq checks a theorem by checking whether its proof script can construct a well-typed proof term for the theorem statement.

In practice, this checking is performed by tools such as \texttt{coqc}, the Coq/Rocq compiler.
Given a \texttt{.v} file, \texttt{coqc} type-checks the definitions, hypotheses, theorem statements, and proof scripts in order.
A theorem is accepted only if the generated proof term is well typed under the formal definitions, assumptions, and imported lemmas available in the current environment.
Therefore, a mechanized proof is machine-checkable: its correctness is validated by the proof assistant's formal type-checking rules, rather than only by human inspection.
In our setting, a final verified proof should compile successfully and should not rely on unfinished proof holes such as \texttt{admit} or \texttt{Admitted}.
\item Coq/Rocq proofs are checked relative to the assumptions available in the current formal environment. The automatic part of this checking is performed by the proof assistant: tools such as coqc verify that the definitions, theorem statements, and proof scripts are well typed, and that the proof script constructs a valid proof term for the stated theorem. However, Coq/Rocq does not automatically judge whether the assumptions themselves are semantically appropriate. Ordinary Hypothesis declarations become explicit preconditions of the theorem, while stronger trusted declarations such as Axiom introduce facts without proof. A theorem proved under such assumptions may still pass coqc, but its trustworthiness depends on whether these assumptions faithfully capture the intended model and are acceptable for the result being proved. Therefore, the verification of a mechanized proof has two layers: the proof script is mechanically checked by Coq/Rocq, while the adequacy of the formalization and the justification of its assumptions are currently inspected by humans, possibly assisted by tools that report remaining axioms, hypotheses, admit, or Admitted.
\end{itemize}

Prosa basic
\begin{itemize}
    \item PROSA is a library of machine-checkable definitions and proofs for real-time schedulability analysis. Its goal is to make real-time scheduling theory more reliable, reusable, and readable by expressing scheduling models, assumptions, and analysis results in Coq/Rocq. Unlike a collection of isolated formal statements, PROSA is designed to resemble the structure and terminology commonly used in real-time systems papers. Its value therefore lies not only in its formal definitions, but also in its reusable lemmas, proof patterns, and proof conventions, which allow new analyses to build on existing mechanized results instead of starting from scratch.
    \item PROSA describes real-time systems through a trace-based view of system behavior. At the lowest level, it introduces abstract entities such as jobs, tasks, time, arrival sequences, and schedules. An arrival sequence specifies which jobs are released over time, while a schedule describes how the system allocates processors to jobs at each time instant. Based on these behavioral objects, PROSA defines semantic notions such as whether a job is scheduled, whether it receives service, whether it completes, and how much workload or interference occurs in an interval. For example, a basic semantic property is that a job can receive service at a time only if it is scheduled at that time. Higher-level timing properties, such as response time and schedulability, are then defined on top of these behavioral notions. In this way, PROSA organizes real-time scheduling concepts from basic system behavior to derived analysis properties.
    
    \item A key feature of PROSA is that its results are highly parameterized. Instead of fixing one concrete task set or one concrete scheduler, PROSA usually states lemmas over abstract job and task types, together with functions such as job arrival times, job costs, task deadlines, task periods, arrival sequences, and schedules. The required model properties are stated separately as hypotheses, such as assumptions about task validity, arrival behavior, or scheduling policy. As a result, a high-level theorem in PROSA is not tied to a single implementation; it can be instantiated for any concrete system that provides the required objects and satisfies the required assumptions. This parametric design improves reuse, but it also makes proof construction harder, because applying an existing PROSA lemma often requires identifying the right parameters and proving all of its preconditions.
    \item PROSA proofs also make extensive use of the SSReflect and Mathematical Components proof style. SSReflect is a Coq extension that provides a compact and disciplined tactic language, while Mathematical Components is a large library built around SSReflect with reusable algebraic, finite, and combinatorial structures. This style emphasizes small proof steps, explicit intermediate facts, structured rewriting, boolean reflection, and compact tactics such as move, have, suff, and by. As a result, PROSA proofs often look different from plain Coq proofs based mainly on intros and apply. This proof style improves readability and reuse in large developments, but it also introduces specific proof-engineering issues, such as managing local subgoals created by have or expanding compressed by ... scripts when they fail.
    \item A Coq/Rocq development is usually organized as a collection of files and modules, rather than as a single self-contained proof file. An import is a command that loads previously defined content from another Coq/Rocq file or library into the current file. For example, after importing a PROSA module, the current proof may use the definitions, notations, tactics, and lemmas provided by that module, as long as their names are accessible in the current namespace. These imported objects become part of the proof environment: they can be used in theorem statements, applied during proofs, or inspected through commands such as Check, Search, and Print, usually issued through tools like coqtop or language-server interfaces. This is particularly important for PROSA, where new proofs are expected to reuse existing definitions and lemmas from the library instead of redefining them locally. Therefore, effective proof construction often depends on importing the right modules, finding the right library lemma, and instantiating it correctly in the current context.
\end{itemize}


}
\rtc{
\begin{itemize}
    \item Rocq Toolchain consists of several components serving different purposes. Rocqc is the batch compiler responsible for parsing and verifying Rocq files while Rocqlsp (Rocq Language Server Protocol), providing standardized interfaces including proof goal feedback, type information and error diagnostics.
\end{itemize}
}
\guan{tactics: }

\guan{proof\_region}

\subsection{Prosa Basics}


\guan{
\begin{itemize}
    \item say prosa's good readability feature is helpful to automated proving
    \item the hierarchy of Prosa. model, analysis, and so on, this is useful because later in experiment w/o full prosa ... 
    
    \item parametric nature of Prosa.
\end{itemize}
}


\guan{JUNYI: write a paragraph about the hierarchy of Prosa: }
Porsa v0.6
\begin{itemize}
     \item classic.util: The namespace collects shared utilities, proof tactics, and reusable lemmas on sequences, counting, fixed points, arithmetic, and other generic proof infrastructure. This is a support layer used throughout the classic development.
    \item prosa.behavior: The namespace collects basic definitions and properties of system behavior (i.e., it defines Prosa’s trace-based semantics). There are no proofs here. 
    \item prosa.model: The namespace collects all definitions and basic properties of various system models (e.g., sporadic tasks, arrival curves, various scheduling policies, etc.). There are only few proofs here. This module contains multiple alternatives of the same concept (e.g., periodic vs. sporadic tasks, uni- vs. multiprocessor models, constrained vs. arbitrary deadlines, etc.), and higher-level results are expected “pick and choose” whatever definitions and assumptions are appropriate.model
    \item prosa.analysis: The namespace collects all definitions and proof libraries needed to establish system properties (e.g., schedulability, response time, etc.). This includes a substantial library of basic facts that follow directly from the trace-based semantics or specific modelling assumptions. 
    \item prosa.results: The namespace contains all high-level analysis results.results
    \item prosa.implementation: Concrete implementations of some of the axiomatic models to which the results apply.
    \item prosa.implementation.refinements: The refinements needed by POET to compute with large numbers, based on CoqEAL.
\end{itemize}

Prosa v0.4
\begin{itemize}
    \item classic.util: The namespace collects shared utilities, proof tactics, and reusable lemmas on sequences, counting, fixed points, arithmetic, and other generic proof infrastructure. This is a support layer used throughout the classic development.

\item classic.model: The namespace collects the core definitions of the classical Prosa development, including time, arrivals, schedules, priorities, suspension models, and schedulability-related notions. In contrast to prosa0.6, this namespace also contains much of the basic trace-based semantics that later became separated into prosa.behavior, together with some local lemmas and basic properties.

\item classic.analysis: The namespace collects most proof developments of the classic library. It is organized by platform and assumptions, such as uniprocessor, global multiprocessor, and APA settings, with further variants for jitter, arrival curves, or suspension. This namespace contains both low-level proof libraries and many high-level analysis theorems, so it plays the role of both prosa.analysis and a large part of prosa.results.

\item classic.implementation: The namespace contains concrete instantiations of the abstract models, such as concrete tasks, jobs, and arrival sequences, as well as executable examples used by the analyses.
\end{itemize}
An example of lemma in classic.model. This establishes the fundamental fact that an entity cannot receive service without being scheduled.
\begin{figure}   
  \centering          
  {
      \includegraphics[width=0.48
      \textwidth]{lemma_in_model.png}
  }
  \caption{An example of a classic.model} 
        
\end{figure}
An example of lemma in classic.analysis. This proves that the interference bound under EDF scheduling is monotonically increasing with the time window.
\begin{figure}   
  \centering          
  {
      \includegraphics[width=0.48
      \textwidth]{lemma_in_analysis.png}
  }
  \caption{An example of a classic.analysis} 
        
\end{figure}



\subsection{LLM-based Agents}


==> sections/backup.tex <==
\subsection{Enhancing PROSA Benchmark for Formal Proofs}

Benchmark enhancements have been explored in prior works to enrich 
the dataset available \begin{enumerate*}
    \item  as evaluation samples or 

    \item as reasoning references for LLMs to learn from.
\end{enumerate*}
This approach has shown improvement in the performance of LLMs 
in various tasks\cite{rocqstar},

Cerqueira et al.\cite{prosa} introduced PROSA, a flexible, open-source and extensible 
foundation for formally proven schedulability analyses that aims at enabling 
formal verification.
These analyses are formalized in the Coq proof assistant, providing a solid knowledge base
from related papers and a composition framework for real-time schedulability definitions,
simple theorems and lemmas. 
Thus, many following works\cite{intuition2coq, aRTA, transferschedulability}
have built upon PROSA to develop formal verification frameworks in real-time systems.
Also, works such as Abstract Response Time Analysis\cite{aRTA} have extended PROSA with 
abstract models to enable more general formal verification along with detailed proofs 
both in formal methods and mathematics.

To systematically evaluate theorem-proving capabilities, we constructed a benchmark dataset derived from the PROSA (Formally Proven Schedulability Analysis) library\cite{prosa}. To establish a structured gradient of difficulty, we categorized the theorems and lemmas within the PROSA corpus based on their proof dependency depth.

We define a recursive stratification scheme for this classification: a theorem or lemma whose proof relies on no other established theorems or lemmas within the library is classified as Level 0. Subsequently, a theorem is assigned Level n if the maximum level of any theorem or lemma invoked within its proof is n-1. Applying this metric, we processed the PROSA library and successfully stratified the constituent proofs into 15 distinct hierarchical levels.

Following this classification, we isolated each theorem and lemma into individual test files to serve as independent evaluation instances. To ensure the models or provers are evaluated strictly on the target proof, all original proofs were excised from the core environment. This methodology yields a comprehensive, level-graded benchmark suitable for assessing automated reasoning across varying degrees of logical complexity.


\begin{table}[htbp]
\centering
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Agent} & \multicolumn{4}{c}{Tactic Length} \\
\cmidrule(lr){2-5}
 & 1-20 & 21-40 & 41-60 & 61+ \\
\midrule
Group size & -- & -- & -- & -- \\
\midrule
RocqStar & -\% & -\% & -\% & -\% \\ % proving agent
Copilot & -\% & -\% & -\% & -\% \\ % commercial agent
Opencode & -\% & -\% & -\% & -\% \\ % Our Baseline
\textbf{Our} & \textbf{-\%} & \textbf{-\%}& \textbf{-\%} & \textbf{-\%} \\
\bottomrule
\end{tabular}
\caption{Evaluation on PROSA, sorted by Tactic Length}
\label{tab:ablation}
\end{table}


\color{red} At least do paper reading ablation. \color{black}

\begin{table}[htbp]
\centering
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Agent} & \multicolumn{2}{c}{Benchmark} \\
\cmidrule(lr){2-3}
 & PROSA & Case Study \\
\midrule
Group size & 100 & 37 \\
\midrule
\textbf{Our} & \textbf{-\%} & \textbf{-\%}  \\
Our w/o Paper Reading & -\% & -\%  \\ % must do, minimum
Our w/o Tools & -\% & -\% \\
Our w/o Expert Skills & -\% & -\% \\
OpenCode Raw  & -\% & -\% \\
ChatGPT 5.4 & -\% & -\%  \\
\bottomrule
\end{tabular}
\caption{Ablation study}
\label{tab:ablation}
\end{table}




\guan{
\begin{itemize}
\item reviewer and writer are identical except the prompt
\item "approve": (1) coqc compile (2) reviewer thinks it's ok. 

\item reviewer read the compile report generated by coqc

\item writer: write --> call coqc --> see if pass or not, if not, writer will revise or not?  TO BE CONFIRMED BY JUNYI

\item writer: we instruct the write to do the following

\begin{itemize}
\item Decompose the semantics: it's unclear what is output.

\item we ask it to do three subtasks:

\begin{itemize}
\item subtask 1: select ".v" files () from prosa, which includes, variables, definitions, hypothesis. definitions does not need to be written explicitly, 
(the range of variables and hypothesis is that particular file, but the range of definitions is global), variables and hypothesis needs to be rewritten in the current .v file. 

(teach the LLM what should be modeled as variables, definition and hypothesis: )


\item subtask 2: model the variables, definitions, hypothesis which are needed but not provided in Prosa. 

\item subtask 3: write the lemma statement


\end{itemize}

\end{itemize}

\end{itemize}

}
\begin{comment}
\paragraph{Instance structure.}
Each instance contains:
\begin{itemize}
    \item a target paper or paper excerpt;
    \item one or more input \texttt{.v} files;
    \item the relevant Prosa classic model fragment;
    \item for the Hybrid setting, a curated assumption-bank document;
    \item a human-reviewed gold assumption set.
\end{itemize}

%%\paragraph{Dataset split.}
%%All methods are evaluated on the same instances. Because our goal is comparative evaluation rather than predictive generalization to unseen labels, we do not introduce a train/dev/test split in the traditional machine learning sense. Instead, we treat the dataset as an evaluation benchmark and report per-instance results aggregated over all instances. If prompt tuning or assumption-bank construction requires development instances, these must be separated and reported explicitly.\footnote{In the final version, we will specify whether any instances were used during prompt development.} 

\subsection{Gold Standard and Annotation Protocol}
\label{subsec:gold}

For each instance, the gold standard is a \emph{human-audited assumption set}.
The gold set is not merely a list of accepted assumptions, but also includes metadata describing the role and status of each assumption.

Each assumption in the gold annotation is labeled as one of the following:
\begin{itemize}
    \item \textbf{E} (\emph{explicit}): explicitly stated in the paper or directly inherited from the formal model reference;
    \item \textbf{I-N} (\emph{implicit-necessary}): not stated verbatim, but necessary for faithful modeling or for the proof to go through;
    \item \textbf{I-O} (\emph{implicit-optional}): a reasonable and acceptable modeling choice, but not clearly necessary;
    \item \textbf{T-S} (\emph{too-strong}): stronger than what the paper justifies;
    \item \textbf{C} (\emph{conflicting/hallucinated}): unsupported, contradictory, or fabricated.
\end{itemize}

For Dataset~1, we additionally distinguish assumptions that are known to be \emph{proof-necessary}, based on the completed formal proof.

\paragraph{Annotation process.}
Each instance is reviewed by a human annotator with knowledge of both the paper and the Coq formalization.
The annotator inspects the paper, the Prosa model fragment, and the input \texttt{.v} files, and then constructs a reviewed assumption set.
For Dataset~1, the annotator also checks the completed proof to identify assumptions known to be necessary for proof completion.

\paragraph{Equivalence of assumptions.}
A major open issue is semantic equivalence between differently phrased assumptions.
Two assumptions may differ syntactically but play the same semantic role.
In the current version, we leave this as an open methodological issue and perform matching at the human-audited semantic level rather than by exact string match.
We plan to formalize equivalence classes of assumptions in future work.
\textbf{Question/TODO:} define a principled equivalence relation for natural-language and Coq-level assumptions.

\subsection{Baselines and Comparison Groups}
\label{subsec:baselines}

We compare the following four conditions.

\paragraph{Generate-only.}
The LLM receives the paper PDF, the input \texttt{.v} files, and the relevant Prosa model fragment, and generates missing assumptions directly without an assumption bank.

\paragraph{Hybrid.}
The LLM receives the same inputs as above, plus an assumption bank.
It is instructed to first select assumptions from the bank and only introduce new assumptions when the bank does not cover the needed semantics.

\paragraph{Human-only.}
A human expert performs the assumption-modeling task from scratch, without any LLM assistance.

\paragraph{Human + Hybrid.}
A human expert reviews and edits the output produced by the Hybrid system.
This condition is used to measure whether LLM assistance reduces human effort while preserving modeling quality.

\paragraph{Why these baselines?}
Generate-only isolates the unconstrained generation ability of the LLM.
Hybrid tests whether a controlled candidate space improves quality and auditability.
Human-only provides the unaided expert-effort baseline.
Human + Hybrid captures the intended human-in-the-loop usage scenario.

\subsection{Experimental Protocol}
\label{subsec:protocol}

For each instance, we run the selected method and collect:
\begin{itemize}
    \item the revised \texttt{.v} file;
    \item the full list of adopted assumptions;
    \item evidence for each assumption, including whether it was selected from the bank or newly added;
    \item wall-clock generation time;
    \item in human-in-the-loop settings, human review time and edit operations.
\end{itemize}

    

\paragraph{LLM prompting.}
The prompting protocol instructs the model to:
\begin{itemize}
    \item treat the paper as the primary semantic source;
    \item treat Prosa as the primary formalization reference;
    \item modify the \texttt{.v} file conservatively;
    \item distinguish model assumptions, data-structure assumptions, and proof-related assumptions;
    \item in the Hybrid setting, prefer bank selection over free generation.
\end{itemize}

\paragraph{Human review protocol.}
For Human + Hybrid, the reviewer is shown the LLM-produced assumptions, their evidence, and the revised Coq file.
The reviewer may accept, delete, rewrite, or add assumptions.
We log:
\begin{itemize}
    \item review time;
    \item number of accepted assumptions;
    \item number of deleted assumptions;
    \item number of rewritten assumptions;
    \item number of newly added assumptions by the human reviewer.
\end{itemize}

\paragraph{Repeated runs.}
If stochastic decoding is used, each LLM condition should be run multiple times per instance and we report mean and variance.
In the current setup, unless otherwise stated, we use a fixed prompt and fixed decoding configuration.
\textbf{TODO:} specify temperature, model version, and number of runs.

\subsection{Evaluation Metrics}
\label{subsec:metrics}

We evaluate methods along six dimensions.

\subsubsection{Acceptable Precision}
\label{subsubsec:precision}

We define \emph{acceptable precision} as the fraction of output assumptions that are acceptable after human audit:
\begin{equation}
\mathrm{AccPrec} = \frac{E + I\text{-}N + I\text{-}O}{N_{\mathrm{out}}},
\end{equation}
where $N_{\mathrm{out}}$ is the total number of output assumptions, and $E$, $I$-$N$, and $I$-$O$ are the numbers of assumptions classified into those categories.

This metric rewards assumptions that are either explicitly justified or acceptable as implicit assumptions, even if they are not strictly necessary.

\paragraph{Human-Baseline Coverage.}
Let $A_{\mathrm{human}}$ denote the set of assumptions constructed by the human baseline, and let $A_{\mathrm{accepted}}$ denote the subset of a method's output that is accepted after human audit. We define Human-Baseline Coverage as
\[
\mathrm{HBC} = \frac{|A_{\mathrm{accepted}} \cap A_{\mathrm{human}}|}{|A_{\mathrm{human}}|}.
\]
This metric measures how much of the human-authored assumption set is covered by the assumptions produced by a method and accepted during audit.

\subsubsection{Over-Strengthening Rate}
\label{subsubsec:strong}

We define the \emph{over-strengthening rate} as
\begin{equation}
\mathrm{StrongRate} = \frac{T\text{-}S}{N_{\mathrm{out}}},
\end{equation}
where $T$-$S$ is the number of assumptions judged stronger than what the paper justifies.

This metric is important because stronger assumptions may make proofs easier while reducing faithfulness to the original paper.

\subsubsection{Hallucination Rate}
\label{subsubsec:hall}

We define the \emph{hallucination rate} as
\begin{equation}
\mathrm{HallRate} = \frac{C}{N_{\mathrm{out}}},
\end{equation}
where $C$ is the number of unsupported, conflicting, or fabricated assumptions.

This metric penalizes assumptions that are neither justified by the paper nor required by the model.

\subsubsection{Necessity Recall (Dataset~1 only)}
\label{subsubsec:necessity}

For Dataset~1, where proof-necessary assumptions are known, we measure whether the method recovers assumptions that are actually required by the completed proof.

Let $G_{\mathrm{nec}}$ denote the set of gold assumptions known to be necessary for the proof, and let $P$ denote the set of predicted assumptions after semantic matching.
We define
\begin{equation}
\mathrm{NecRecall} = \frac{|P \cap G_{\mathrm{nec}}|}{|G_{\mathrm{nec}}|}.
\end{equation}

This metric is only applicable to Dataset~1.
For Dataset~2, necessity cannot be evaluated because the proof is not completed.

\subsubsection{Human Cost}
\label{subsubsec:human-cost}

We evaluate the human effort required under different settings using:
\begin{itemize}
    \item \textbf{time cost}: total human time per instance;
    \item \textbf{edit cost}: number of deletions, rewrites, and additions;
    \item \textbf{acceptance rate}: proportion of model-produced assumptions accepted without modification.
\end{itemize}

For Human-only, time cost corresponds to modeling from scratch.
For Human + Hybrid, time cost corresponds to auditing and editing the LLM output.

We also report \emph{effort reduction}:
\begin{equation}
\mathrm{EffortReduction} = \frac{T_{\mathrm{HumanOnly}} - T_{\mathrm{Human+Hybrid}}}{T_{\mathrm{HumanOnly}}}.
\end{equation}

\subsection{Secondary Analyses}
\label{subsec:secondary}

In addition to the core metrics above, we plan the following secondary analyses.

\paragraph{Bank utilization.}
For the Hybrid method, we measure:
\begin{itemize}
    \item the number of assumptions selected from the bank;
    \item the number of assumptions newly added outside the bank;
    \item the rejection rate of bank items that were considered but not adopted;
    \item the fraction of accepted assumptions that came from the bank.
\end{itemize}

\paragraph{Category-wise performance.}
We separately report results for:
\begin{itemize}
    \item model assumptions,
    \item data-structure assumptions,
    \item proof-related assumptions.
\end{itemize}
This helps identify whether LLM assistance is more reliable for modeling semantics than for proof-specific technical side conditions.



\subsection{Statistical Reporting}
\label{subsec:stats}

For each metric, we report the mean and standard deviation across instances.
When comparing methods, we will use paired statistical tests when appropriate, since all methods are evaluated on the same set of instances.
\textbf{TODO:} choose the final significance test (e.g., paired $t$-test or Wilcoxon signed-rank test) depending on the observed metric distributions.
\end{comment}


\subsection{Datasets}
\label{subsec:datasets}

We construct two datasets.

\guan{each item in the dataset consists the natural language and the human written formalization. the checking between the human written formalization and the LLM generated one is checked by using the coq (manually) proving their equivalence}


\paragraph{Dataset~1: proof-completed benchmark.}
This dataset contains 20 instances collected from Prosa and manually constructed theorems.
For each instance, the proof has already been completed, and the assumptions required by the proof are known.
This dataset enables evaluation of \emph{necessity}, because one can compare the generated assumptions against assumptions known to be required by the completed proof.

\paragraph{Dataset~2: modeling-only benchmark.}
This dataset contains \texttt{xx} instances, manually constructed from papers and Coq modeling artifacts for which modeling assumptions are available but the corresponding proofs are not completed.
This dataset supports evaluation of modeling faithfulness and human usefulness, but not proof-level necessity.
In other words, for Dataset~2, we can evaluate whether the assumptions are acceptable for modeling, but we cannot reliably determine which assumptions are strictly necessary for a finished proof.


% \subsection{Agentic Workflow for PROSA Benchmark Proof Generation}
% To effectively utilize LLMs for generating formal proofs within the PROSA framework,
% we design an agentic workflow that enables dynamic proof strategy generation that fully 
% leverages the strengths of LLMs in formal reasoning and proof synthesis.

% \subsubsection{Reasoning Guidance for PROSA Proof Generation}

% The agentic workflow begins with the identification of the proof goal within the PROSA framework.
% The LLM is provided with the enhanced PROSA benchmark, including the curated theorems 
% and their natural language descriptions. Using this information, the LLM generates a 
% high-level proof strategy, outlining the steps required to achieve the proof goal.
% This strategy serves as a roadmap for the subsequent proof generation process.

% \subsubsection{Tool Calling and Agent Skills Integration}

% To facilitate the proof generation process, we integrate tool calling capabilities and agentic 
% skills including interface with Coq to acquire current states and procedural knowledge of fetching
% and understanding relevant lemmas and theorems from the PROSA library.



\subsection{Experiment For Task 2}

% There are two main experiments for task 2: 
% First, process PROSA into a benchmark with a size of 1000+ theorems and lemmas and ask all agents and proving models to test on benchmarks. (Given Definition and Hypothesis based PROSA and complete PROSA)
% Second, use Case study with all PROSA to test the agents with capability of retriving external knowledge. (Given complete PROSA)

To evaluate the performance of our agent systems with the current ones, we split the experiments into two sub-tasks.

\subsubsection{PROSA Benchmark}
As stated in \ref{}, we have processed PROSA as a test benchmark to test the proof generation capabilities of different agents in the aspect of real-time scheduling.
The experiment conditions are set as follows: First 







\subsubsection{Case Study}
To assess the effectiveness of our agent in formalizing previously unverified results, we construct a benchmark consisting of 37 theorems and lemmas. These are manually formalized from nine real-time scheduling conference papers and one textbook, all of which are not currently proven in PROSA.

We compare the following configurations:
\begin{itemize}
    \item RocqStar
    \item OpenCode
    \item \ours\
\end{itemize}



\guan{version 1:}

A fundamental difference between automated theorem proving (ATP) for real‑time scheduling theory and ATP for pure mathematics lies in the sheer scale and complexity of the formal statements involved. In popular LLM evaluation benchmarks for mathematics, such as PutnamBench \cite{}, lemma descriptions—including necessary definitions and local hypotheses—typically range from 100 to 1,000 lines. In stark contrast, the lemmas that arise in schedulability analysis are an order of magnitude larger. For example, stating the main schedulability theorem from \cite{} in its full formal context, incorporating all dependent definitions, variable declarations, modeling assumptions, and the theorem statement itself, requires 5,620 lines of Lean code. An LLM-based prover must therefore reason over exceedingly long and information‑dense proof contexts, far beyond what current systems are routinely tested on.

This extraordinary length is not mere verbosity; it is a direct consequence of the modular and deeply conditional structure of scheduling libraries. The Prosa library \cite{} is carefully architected so that lemmas can be reused across different task models, scheduling policies, and execution platforms. As a result, whether a given library lemma can be invoked in a new proof is governed by a cascade of preconditions. Those preconditions depend in turn on other preconditions, and the chain eventually bottoms out in model‑specific hypotheses—such as whether tasks are sporadic or periodic, whether preemptions are allowed, or whether certain arrival curves are respected. The same lemma may be applicable in one model and invalid in another, and an ATP agent cannot simply match a lemma’s conclusion to a goal. It must autonomously navigate a vast, conditional proof graph where every inference step is contingent on a web of assumptions that change from problem to problem. This makes proof search qualitatively harder than in many mathematical domains where the ambient context is more stable.

Compounding these intrinsic difficulties is a severe scarcity of domain‑specific training data. The theorem‑proving capabilities of state‑of‑the‑art LLMs are largely acquired during pre‑training on massive corpora of formalized mathematics, such as Mathlib \cite{}. Public data for mechanized schedulability analysis, however, is extremely rare. Prosa represents virtually the only such resource, and its total volume is orders of magnitude smaller than the Lean mathematical corpus. An LLM therefore enters this domain with minimal exposure to scheduling concepts, notation, and proof patterns, unable to fall back on patterns absorbed from millions of mathematical proofs. The agent must simultaneously cope with enormous proof obligations, intricate conditionality, and a near‑vacuum of learned scheduling‑specific heuristics.

Thus, LLM-based ATP for real‑time scheduling faces a unique confluence of challenges: vast, densely interdependent proof contexts that arise from a library designed for cross‑model reuse, and a drastic lack of pre‑training data that would otherwise allow a model to internalize the domain’s structure. Any effective LLM‑agent approach must explicitly address this combination.

% We also need ablation study, minimum is to test w/o paper instruction
% we also should do more ablation study if possible: 
% (Our subagent, Our tools, Our exprt knowledge)


First, 
the proof of schedulability analysis requires particular expertise in proving real-time scheduling theory (e.g., some particular concepts, abstractions, and proving tricks). Although existing LLM already has good general knowledge in real-time scheduling, its knowledge in such real-time scheduling specific knowledge are relatively much weaker.
Second,The lengthy lemma description leads to challenges in not only 
proving the lemma, but also make it already very challenging to formalize the theorems. Third, the structure of Prosa introduces challenges in its proof. Prosa is developed to serve as a common foundation for a wide range of schedulability analysis problems, so many concepts Prosa 

\ours\ consists of two main components. The first component, \oursformal, assists users in generating formalized lemma statements in Rocq. The second component, \oursprove, helps users automatically generate correct proofs for the lemmas verified by Rocq. 


\guan{my writing ends here!!!!!!!!!!}

Recently there have been many LLM-base agent systems for automated theorem proving for solving mathematic problem, their performance in generating \guan{formalization??} proofs in real-time schedulability analysis domain is quite poor (as will be seen in the evaluation of Section \ref{}). This is because the schedulability analysis has some unique features different from the targeting domain of these existing tools (e.g., pure mathematics problems).
In mathmatics 


\item Guiding Principles for Decomposition : The decomposition process adopts a two-stage approach: first, a semantic-level decomposition guided by the core mathematical reasoning, followed by a syntactic-level decomposition tailored to be Rocq-friendly. Specifically, the semantic decomposition analyzes the source paper or the immediate theorem context to extract the fundamental steps that genuinely advance the mathematical proof. Subsequently, the syntactic decomposition bridges the mechanization gap, enabling Rocq to successfully verify the proof. This involves necessary operations such as representation transformations, index manipulations, lemma alignments, and the discharging of residual arithmetic goals. Furthermore, we outline several common transformations utilized during the semantic-level decomposition:

\begin{itemize}
    \item \textbf{Shape Transport (\texttt{shape\_transport}):} This transformation aligns the structural representation of a term with the prerequisites of an applicable lemma. For instance, suppose the goal is to prove that the number of objects satisfying a given condition is at most $1$. If the current context provides the hypothesis $\texttt{size (filter P xs)} \le 1$, but the available lemma strictly requires the premise $\texttt{count P xs} \le 1$, a \texttt{shape\_transport} step is necessary to transform the hypothesis from $\texttt{size (filter P xs)} \le 1$ into $\texttt{count P xs} \le 1$.

    \item \textbf{Witness Transport (\texttt{witness\_transport}):} This transformation handles existential instantiations and their associated properties. For example, consider a goal requiring the proof that there exists a job $j$ that falls within a specific interval and belongs to a task $tsk$. Through \texttt{witness\_transport}, this existential goal is decomposed by instantiating a concrete witness $j$ and explicitly extracting its two requisite premises: the job $j$ lies within the designated interval, and $j \in tsk$.
    \item .....
\end{itemize}



However, the soft-constraint nature of prompting faces a very important challenge to realizing this decomposition-oriented architecture: when we assign a goal to an agent, we want it to try its best to prove the lemma directly, and only decompose it if it truly cannot make progress. In practice, however, we observe that as long as the agent has the option to decompose a goal, it tends to default to decomposition after only a few failed attempts. Worse still, the decomposition it produces is often trivial, genuinely making no progress. The result is a cascade where the main agent decomposes a lemma only to have each subagent recursively decompose its own subgoals, all the way down the hierarchy, and no agent actually solves anything. We refer to this phenomenon as the lazy agent problem—a well‑known pathology in multi‑agent systems, where agents shirk responsibility and shift work downward to avoid effort. We have tried very hard to tune the prompt, but this problem still exists to some degree. Note that this problem is not because we let the same agent to both can prove and can choose to decompose. The problem fundamentall still exist even if we define two types of agents, one dedicated to decomposition and one dedicated to proving, because the problem fundementally is because we rely on the LLM's decision to decide when to give up 

To address this problem, we choose to add external 



We define two types of agents: decomposing agents (D-Agents) and proving agents (P-Agents).
\begin{itemize}
\item \textbf{D-Agent}: decomposing a lemma into a set of sub-goals. 
\item \textbf{P-Agent}: proving a goal completely. 
\end{itemize}
Our system first decomposes the lemma into subgoals, then proves each one. If a P-Agent fails to prove its assigned subgoal within the iteration limit, the system spawns a new D-Agent to decompose that subgoal further. This process recurses until the subgoal is proved or the timeout is reached.
Figure \ref{} illustrates this procedure. Conceptually, D-Agents and P-Agents may be recursively generated for an arbitrary number of levels. In practice, however, the recursion depth is typically small (e.g., 2–3 levels), since lemmas are either proved successfully or terminated due to timeout before reaching deep recursion.


Both types of agents aim to produce a proof that passes verification by the verifier—an external tool (the coqc engine plus extra checking scripts; see Section \ref{}) that checks whether a proof correctly establishes the lemma. The difference is that, a D-Agent may complete a proof with unsolved subgoals, whereas a P-Agent must produce a complete proof without unsolved subgoals. These unsolved subgoals become the goal for a P-Agent to solve (or, if the P-Agent fails, they trigger further decomposition at the next recursion level).


To enforce this fine-grained exploration, the prompt instructs the sub-agent to execute only a single minimal tactic or a short tactic block at a time. Following each step, it must immediately inspect the resulting proof state---specifically the updated goals and hypotheses. 
Once a step is deemed effective, the agent is required to checkpoint this state to facilitate future backtracking. Conversely, in the event of a failure, the agent must refrain from a monolithic rewrite of the entire proof script, and instead isolate the exact locus of the first error to diagnose the precise bottleneck. Furthermore, any external knowledge retrieval must be strictly constrained to the specific missing artifact that directly addresses this immediate sticking point.


\paragraph{Rocq Proof Methodology.}
This skill serves as the foundational operating protocol of the agent. Its purpose is to ensure that proof construction remains synchronized with the live proof state rather than with a speculative multi-step plan. Concretely, it enforces a one-step-at-a-time discipline: the agent executes a single tactic, inspects the resulting goals, and only then decides the next step. The skill also prioritizes errors according to semantic severity, giving precedence to parsing failures, typing errors, and tactic failures before stylistic cleanup. In addition, it prescribes structured subgoal management through bullets and braces, advocates working on the hardest case first while temporarily admitting less critical branches, and provides a principled automation hierarchy for tactics such as \texttt{reflexivity}, \texttt{lia}, \texttt{ring}, \texttt{tauto}, and \texttt{auto}. Overall, this skill acts as a proof-hygiene layer that prevents the agent from producing long but semantically disconnected scripts.


\paragraph{Coq Proof-State Discipline.}
This skill is a syntax-aware normalization procedure for situations in which a rewrite appears mathematically justified but fails syntactically in Coq. It is designed for proof branches that oscillate among ssreflect big operators, iterated addition, multiplication, and boolean-as-natural encodings. Its core rule is that the next lemma must be selected from the exact surface form of the current goal, not from the intended mathematical destination alone. If the left-hand side of a desired lemma is not a literal subterm of the goal, the agent is instructed not to rewrite immediately; instead, it must first insert a small bridge lemma or perform a local normalization step that converts the goal into a compatible form. The skill therefore promotes inside-out normalization, branch-local bridge lemmas, and commitment to a single stable normal form instead of repeated movement between extensionally equivalent representations. This substantially improves robustness in ssreflect endgames involving lemmas such as \texttt{big\_const\_ord}, \texttt{iter\_addn}, and \texttt{mulnC}.

\paragraph{Ssreflect Count Bridging.}
This skill specializes the previous normalization discipline for counting arguments in MathComp/ssreflect. It is triggered when the same quantity appears in multiple interchangeable forms, such as an indicator sum of the form \texttt{if P x then 1 else 0}, a filtered big operator, a \texttt{count}, and eventually an arithmetic or \texttt{min}-based bound. The skill imposes a strict monotonic normalization pipeline: first convert the indicator sum into a filtered big operator, then collapse the filtered sum of ones into a \texttt{count}, then establish a bound on that count, and only afterwards perform the final arithmetic or \texttt{min} reasoning. A further contribution of this skill is its explicit separation between the boolean layer and the Prop layer. Once the branch reaches a stable count expression, the agent is encouraged to cross from boolean reflection into Prop arithmetic exactly once and then remain there for the rest of the argument. This specialization is important because count-based branches require not only normalization, but normalization toward the correct semantic layer.


In our agent system, proof-repair skills are selected according to explicit failure signature observed in the proof state.
Rather than treating skills as broad annotations, the system associates each skill with a well-defined class of proof failures.


The skill library is organized into six \color{red}layers\color{black}. \emph{Rocq Proof Methodology} provides the global operating discipline of the agent. \emph{Goal Focus Discipline} and \emph{By Expansion Diagnostics} recover trustworthy structural information when compact proof scripts or branching tactics obscure the real proof state. \emph{Coq Proof-State Discipline} and \emph{Ssreflect Count Bridging} address representation mismatches by enforcing controlled normalization toward stable forms. Finally, \emph{Coq Goal-Driven Apply for Early-Bound Arguments} regulates theorem application in cases where implicit parameters, section binders, or typeclass instances must be fixed before ordinary proof obligations can be generated.


\paragraph{By Expansion Diagnostics.}
This skill is a debugging procedure for compact ssreflect scripts that fail on a \texttt{by} line with a flat message such as ``No applicable tactic.'' The key insight is that \texttt{by} is not a substantive proof method in itself; rather, it is a compression boundary that suppresses intermediate proof states by requiring the payload tactic to solve all generated goals immediately. As a result, when a \texttt{by} line fails, the visible error often hides the true cause, which may be an extra branch, an unfinished local subgoal, a rewrite mismatch, or an incorrect theorem application. The skill therefore instructs the agent to remove only the \texttt{by}, replay the exact same payload, and treat the first newly exposed proof state as the true diagnostic signal. That revealed state then determines which other skill should take over. Structural errors trigger goal-focus recovery, rewrite mismatches trigger syntax-aware normalization, and incomplete local goals are solved directly. This skill is especially useful because human Coq proofs often use compressed idioms for elegance, whereas an automated agent requires explicit intermediate states for dependable debugging.


Taken together, these skills form a layered control architecture rather than a flat collection of prompts. The guiding principle is not to search for arbitrary tactics, but to recognize recurrent proof situations and attach to each situation a bounded and interpretable recovery or progress procedure. This makes the agent easier to analyze, easier to debug, and more reliable in long Coq developments, especially in ssreflect-heavy proofs where structural drift and representation mismatch are common.


\begin{itemize}

\item \textbf{Normal-form selection and bridge order.}
First determine whether the endgame is about \texttt{count} or a big-operator identity.
Once a primary normal form is chosen, move monotonically along the chain
indicator sum $\to$ filtered big operator $\to$ count,
and avoid oscillating between representations.

\item \textbf{Count bounds before min/arithmetic.}
Stabilize the core fact as a bound on \texttt{count} first, and only then derive
results about \texttt{Nat.min}, \texttt{minn}, or the final inequality.
Do not start the arithmetic endgame while the counting representation is still unstable.

\item \textbf{Bool/Prop boundary management.}
If the branch will need \texttt{lia} or a side condition for \texttt{Nat.min},
reflect the relevant boolean inequality into Prop exactly once and finish the rest
of the branch in the Prop layer.
Reflect back only if the final goal itself is boolean.

\item \textbf{Failure signals and anti-patterns.}
When \texttt{big\_mkcond} or \texttt{sum1\_count} does not match, the branch is usually
not yet in the required normal form.
A common anti-pattern is to jump directly from an indicator sum to \texttt{count}
or to a \texttt{min} inequality, which causes both rewriting and arithmetic to drift.


\item \textbf{Minimal expansion strategy.}
When a \texttt{by} line fails, remove only \texttt{by} and keep the tactic payload unchanged.
Re-run immediately and record both the first revealed error message and the number of focused goals.
If expansion produces multiple goals, the primary issue is proof structure.
If it reveals a rewrite mismatch, the issue is the current goal shape.
If it reveals \texttt{Cannot apply} or \texttt{No assumption}, the issue lies in the lemma premises or the local context.

\item \textbf{Standard expansion patterns.}
Rewrite compressed forms such as \texttt{by rewrite}, \texttt{by apply:},
\texttt{have \dots by \dots}, and \texttt{case \dots; by \dots}
into explicit proof scripts.
This exposes the exact step that fails or the exact branch that remains open.
After expanding one \texttt{by} boundary, repair that boundary only.
Do not start guessing alternative tactics before reading the first real error,
and compress back into \texttt{by} only after the expanded script closes reliably.


\item \textbf{Syntax-driven rewriting.}
Before every rewrite, check whether the left-hand side of the intended lemma
is literally a subterm of the current goal.
If it is not, add a bridge step first instead of rewriting from mathematical intuition alone.

\item \textbf{Local bridge-lemma strategy.}
Use a small local bridge lemma when the mismatch is specific to the current branch
or to a fixed local expression.
Extract a generic lemma only when the same normalization gap recurs across proofs.

\item \textbf{Normalization order in big-operator endgames.}
Normalize inner constant sums or boolean-valued sums first,
then perform outer distribution, and only afterward use multiplication-oriented rewrites.
Keep the branch in one stable normal form rather than bouncing among
big operators, \texttt{iter}, and multiplication.

\item \textbf{Failure signatures and skill switching.}
Failures of \texttt{mul1n}, \texttt{mulnC}, or \texttt{big\_ord\_recr}
usually indicate that the goal has not yet reached the required syntactic shape.
Once the branch is clearly about \texttt{count}, \texttt{sum1\_count}, or \texttt{Nat.min},
it should be handled by the count-bridging skill instead.


\item \textbf{Small-step proof construction and goal inspection.}
Write one tactic at a time and inspect the resulting goal state after each step.
This prevents long blind scripts and keeps the real proof state visible.

\item \textbf{Error priority and structured subgoal management.}
Fix syntax and typing errors before addressing tactic failures.
Whenever a proof has multiple subgoals, manage them explicitly with bullets or braces
instead of letting the proof drift structurally.


\item \textbf{Automation and tactic selection strategy.}
Choose tactics from cheaper to more specialized ones, such as
\texttt{reflexivity}, \texttt{lia}, \texttt{ring}, \texttt{tauto},
\texttt{congruence}, \texttt{auto}/\texttt{eauto}, and
\texttt{decide}/\texttt{native\_decide}.
For composite goals, decompose the goal first and automate each component separately.

\item \textbf{Rewriting discipline and management of intermediate facts.}
When dependent rewriting becomes ill-typed, prefer moves such as
\texttt{generalize dependent} or \texttt{subst}.
Use \texttt{assert}, \texttt{pose proof}, and \texttt{set} to name intermediate facts
instead of hiding too much work inside long inline tactic chains.

\item \textbf{Cleanup, proof engineering conventions, and final verification.}
After a proof compiles, clean it up, choose deliberately between \texttt{Qed} and \texttt{Defined},
follow the intended import and Ltac2 conventions, and run an actual compilation check such as \texttt{coqc}.
A proof is not complete until temporary holes such as \texttt{admit} or \texttt{Admitted.} have been removed.


\end{itemize}


%In OpenCode, skills are not injected into the model context merely by being discovered. The system first builds a catalog of available skills by scanning SKILL files from project-local, external-compatible, configured local, and remote registry locations, but this discovery phase only records metadata and content on the runtime side. A skill becomes effective only through an explicit activation path. In the proactive path, the built-in `skill` tool exposes the available skill names and descriptions to the agent; when the agent identifies a match between the current task and a listed skill, it invokes `skill({ name })`, which then returns the full skill body, base directory, and sampled auxiliary files as a structured tool result. In the user-directed path, the TUI presents skills as slash commands, expanding the selected skill body directly into the next user prompt. Coq/Rocq failures add a third, reactive guidance mechanism: proof-related tools append `<coq_skill_hints>` to diagnostic outputs, recommending targeted skills based on failure signatures such as focus drift, compressed `by` scripts, big-operator shape mismatches, or blocked theorem applications. Importantly, these hints do not automatically load a skill; they only influence the agent’s next decision. This design separates skill discovery from skill activation, and further separates error-conditioned recommendation from instruction injection. As a result, skills act less like always-on global prompts and more like task-scoped procedural knowledge that can be deliberately activated when the current proof state justifies it. Context management follows the same principle: loaded skill outputs are preserved by pruning rules, while full-session compaction summarizes historical context without a dedicated “skill completion” lifecycle or automatic unloading step.



\guan{the following i don't understand}
 When the main agent determines that a goal is ready for delegation to a sub-agent, it must first clearly delineate the boundary between this local hole (gap) and the outer main proof. Only after the outer compositional relationships have been explicitly defined can the genuinely local and independent segment be formulated as a proof-region and assigned a stable admit-id to be handed over to the lemma agent. In other words, a delegable region must represent a local obligation with well-defined boundaries and a single responsibility; it must not entangle sub-node syntheses, cross-branch logic, or any massive proof blocks that have not yet completed semantic or shape decomposition.



Any rework process must preserve the previously solved regions that remain compatible. In other words, if a decomposition error is isolated to a single leaf node, the agent should incrementally repair only that specific block and its requisite outer bridging logic, strictly avoiding a complete teardown of the entire proof structure.



\item 7. details : 
 Do not add new section-level, theorem-level, or global assumptions outside the proof.
 Do not replace the proof with a different proof architecture just because it is easier.
 A usable paper proof constrains the semantic spine, but ambiguous or incomplete proof.tex content should be downgraded rather than forced into an unusable Coq split.
First do proof-skeleton generation, then do lemma-by-lemma proving.
 Before any semantic judgment that the theorem is false or the file is wrong, inspect the exact theorem statement, local hypotheses, section or context declarations, imports, and the live Coq goal or hypotheses for completeness.
 Do not leave successful proof code only in conversation; write it back to the file.
 If a proof edit becomes invalid, preserve already validated theorem-level fragments and checkpointed local proof text. Repair by commenting out or moving only the unvalidated failing tail to a scratch note; do not reset a region to an admit or delete validated fragments solely because a later fragment failed.
After enough reading to map the next semantic node or shape-node contract, write the next concrete `pose`, `set`, `have`, `assert`, `suff`, or `enough` step before doing more broad search.
Reading alone is never a deliverable. If the file is still unchanged and you are considering another broad search batch, stop and write the next semantic/shape skeleton step or minimal single-contract admitted placeholder first.


\end{itemize}


\item 3. Proof Guidance: Prior to any formal proof attempt, a concrete, complete, and end-to-end informal proof must be explicitly constructed, which then dictates the trajectory of the formal verification process. 
The sub-agent is permitted to further decompose smaller auxiliary lemmas internally; however, such actions are strictly restricted to localized, single-step decompositions within its assigned \texttt{proof\_region}, centered exclusively around the immediate sub-problem at hand.



\item Escalation to the Main Agent: The system protocol strictly prohibits naive backtracking to the main agent based solely on a minor failure count threshold. Instead, escalation is granted exclusively after a series of sustained interactive proof attempts and must be justified by concrete empirical evidence. These valid indicators of structural escalation include persistently stuck goals, missing premises, repeated synthesis failures of local bridging logic, misdirected goal orientations, overly strong goals, or scenarios necessitating a theorem-level bridge and structural modifications to the outer theorem spine.





\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{ProsaProver26manuscript/sections/agents.jpg}
    \caption{xxx.}
    \label{fig:unify}
    % \vspace{-5pt}
\end{figure}

Each agent wraps a request channel to the backbone LLM. It iteratively sends queries to the LLM via API calls, obtains outputs, and invokes external tools to generate additional information. This feedback loop continues until the agent reaches its target or is terminated upon exceeding the predefined timeout limit.
In each iteration, the agent analyzes the current proof state and determines the next step (e.g., invoking external tools to obtain extra information). The LLM's output, along with any newly generated information, is appended to the query for the next round. \guan{should define the terminology here: context, query, output, external information}. \guan{mention that this is the mainstream way of designing agent, which is friendly to KV cache hit}. \guan{put it in context manager} 



\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]
    {ProsaProver26manuscript/sections/runtime-gpt.png}
    \caption{sample runtime}
    \label{fig:placeholder}
\end{figure}



\rtc{
In our agent system, skills are not incorporated into the model context simply because they are available. Instead, the system adopts a two-stage design that separates skill discovery from skill activation. During discovery, the system constructs a catalog of available skills, recording their names, descriptions, and associated instructional content outside the immediate model context. This catalog serves as an index of procedural knowledge, but it does not by itself affect the agent’s behavior.
A skill becomes operational only when it is explicitly activated. In the proactive activation path, the agent is exposed to the set of available skill descriptions and may select a relevant skill when the current task appears to match its intended use. Once selected, the full instructional content of the skill is introduced as a structured response, allowing the agent to condition its subsequent reasoning on task-specific guidance. 

The system also includes a reactive recommendation mechanism for proof-related failures. When proof checking or proof search fails, diagnostic outputs may include targeted skill hints derived from recognizable failure patterns, such as loss of proof focus, overly compressed proof scripts, mismatches in algebraic or big-operator structure, or blocked theorem applications. These hints do not automatically activate any skill. Rather, they provide contextual recommendations that may inform the agent’s next decision. 
This design treats skills as task-scoped procedural knowledge rather than persistent global prompts. By decoupling discovery, recommendation, and activation, the system avoids unnecessarily increasing the model context while still allowing specialized guidance to be introduced when justified by the task state.
}



The LLM can efficiently generate many useful proving skills, but there are some commom 



Instead of treating Coq theorem proving as a monolithic tactic search problem, our agent relies on a library of specialized skills, each targeting a recurrent failure mode in interactive proof development. Each skill is defined by three components: (i) a trigger pattern extracted from the current proof state or recent diagnostics, (ii) a procedural policy that specifies how the agent should react, and (iii) a local success condition that determines when control can be returned to ordinary proof search. This design replaces unconstrained tactic generation with bounded and interpretable recovery procedures, which improves both reliability and debuggability.



\rtc{


The goal-focus-discipline skill is triggered when the proof state indicates instability in goal focus or branch structure. Typical trigger conditions include errors such as “expected a single focused goal,” “wrong bullet,” “no such goal,” the presence of shelved or unfocused goals, or failures that arise immediately after branching tactics such as case, destruct, split, apply/negP, have, or suff. The skill is also triggered when a branch appears syntactically complete but has only modified a local hypothesis rather than discharging the enclosing goal. These conditions suggest that the main problem is not a missing mathematical lemma, but an ill-structured goal stack. The corresponding repair strategy is therefore to restore bullet discipline, brace structure, and local subproof boundaries before attempting further proof steps.
\guan{notice: here we add hard code.}
}



\guan{what are these transformations: is (\texttt{shape\_transport}) provided by coq/rocq?}
\begin{itemize}
    \item \textbf{Shape Transport:} 
    
    
    
    We instruct the agent to isolate purely representational conversions as independent nodes.
We tell it that when the mathematical content is unchanged, but the current expression must be recast into the exact form
required by a downstream lemma,
that conversion should be marked as a dedicated
\texttt{shape\_transport} step.
Typical examples include conversions among
\texttt{bigop}, \texttt{count}, \texttt{size}, \texttt{filter},
finite-set cardinality, boolean/propositional reflection,
normalized equalities or inequalities, and coercion-adjusted forms.
A simple example is the conversion from
$\texttt{size (filter P xs)} \le 1$ to
$\texttt{count P xs} \le 1$
before applying a counting lemma. \guan{why?}

  \item \textbf{Witness Transport :}
We instruct the agent to make existential or paper-level objects concrete before further proof composition. We tell it that whenever a proof step depends on an object
described only through \texttt{exists}, \texttt{has}, \texttt{pick}, a constructive witness,
or an informal paper-defined entity, it should first introduce an explicit witness
and record the associated membership, interval, ownership, or defining premises as reusable local facts. This conversion should be treated as its own \texttt{witness\_transport} node. A simple example is to turn $\exists j,\; j \in \texttt{jobs\_arrived\_during}\; I \land \texttt{job\_task}\; j = tsk$ into a concrete witness $j$
together with the facts $j \in \texttt{jobs\_arrived\_during}\; I$ and $\texttt{job\_task}\; j = tsk$.
    \item  \textbf{Library Instantiation :}
We instruct the agent to recognize cases where the current proof state already contains the right mathematics, but not yet in the exact syntactic shape required by a Prosa, MathComp, or local lemma. In such cases, we tell it to create a dedicated \texttt{library\_instantiation} node.
Its role is to align parameters, specialize hypotheses, expose side conditions, and match the exact conclusion form expected by the target lemma, without mixing that alignment step with unrelated semantic decomposition. A simple example is to specialize a generic lemma about workload bounds
to a concrete interval $[t_1,t_2)$ and a concrete task $tsk$ before applying it to the current goal.

\item \textbf{Case-Split Boundary:}
We instruct the agent to represent the boundary of a case analysis explicitly,
rather than folding the entire branch proof
into a single local obligation.
We tell it that the role of a
\texttt{case\_split\_boundary} node
is to expose the branch condition
and the branch-local premises
that become available once that condition is assumed,
while leaving the substantive proof
inside each branch
to later nodes.
This teaches the agent
to preserve theorem-level branch structure
instead of over-delegating it.
A simple example is to split on whether
$\texttt{task\_is\_scheduled}\; tsk\; t$
holds at time $t$,
and to record separately
the premises available in the two branches.
\item \textbf{Pointwise Semantic Bridge :}
We instruct the agent to use
\texttt{pointwise\_semantic\_bridge}
when the required semantic connection
must be established one element at a time.
We tell it that this kind of node is needed
when the parent goal is a global counting,
cardinality, or aggregation claim,
but the available semantic argument
naturally yields only a per-element implication.
For example, suppose the parent goal is to prove
\[
\texttt{count (fun j => receives\_service\_in I j) jobs}
\;\le\;
\texttt{count (fun j => arrived\_before (end\_of I) j) jobs}.
\]
We tell the agent not to jump directly
to the counting inequality.
Instead, it should first isolate the local semantic fact
\[
\forall j,\;
j \in \texttt{jobs}
\rightarrow
\texttt{receives\_service\_in I}\; j
\rightarrow
\texttt{arrived\_before (end\_of I)}\; j.
\]
Once this per-job implication has been made explicit,
the later aggregation step can derive
the filtered-list inclusion
or the desired count bound.
\end{itemize}



\begin{table*}[htbp]
\centering
\caption{LLM-generated Proving Skill Summary}
\label{tab:guidelines}
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{
    >{\centering\arraybackslash}p{0.4cm}   % 序号列
    >{\bfseries\raggedright\arraybackslash}p{0.18\textwidth}  % Principle
    >{\raggedright\arraybackslash}p{0.74\textwidth}  % Description
}
\toprule
\multicolumn{1}{c}{\textbf{\#}} & \multicolumn{1}{c}{\textbf{Principle}} & \multicolumn{1}{c}{\textbf{Brief Description}} \\
\midrule
11 & Small-step \& inspect & Write one tactic at a time and inspect the resulting goal state after each step. This prevents long blind scripts and keeps the real proof state visible. \\
\midrule
1 & Normal form \& bridge order & First determine whether the \guan{endgame} is about \texttt{count} or a big-operator identity. Once a primary normal form is chosen, move monotonically along the chain: indicator sum $\to$ filtered big operator $\to$ count. Avoid oscillating between representations. \\
\midrule
2 & Count before min & Stabilize the core fact as a bound on \texttt{count} first, and only then derive results about \texttt{Nat.min}, \texttt{minn}, or the final inequality. Do not start the arithmetic endgame while the counting representation is still unstable. \\
\midrule
3 & Bool/Prop boundary & If the branch will need \texttt{lia} or a side condition for \texttt{Nat.min}, reflect the relevant boolean inequality into Prop exactly once and finish the rest of the branch in the Prop layer. Reflect back only if the final goal itself is boolean. \\
\midrule
4 & Failure signals & When \texttt{big\_mkcond} or \texttt{sum1\_count} does not match, the branch is usually not in the required normal form. Anti-pattern: jump directly from an indicator sum to \texttt{count} or to a \texttt{min} inequality, which causes both rewriting and arithmetic to drift. \\
\midrule
5 & Minimal expansion & When a \texttt{by} line fails, remove only \texttt{by} and keep the tactic payload unchanged. Re-run immediately and record both the first revealed error message and the number of focused goals. If expansion produces multiple goals, the primary issue is proof structure. If it reveals a rewrite mismatch, the issue is the current goal shape. If it reveals \texttt{Cannot apply} or \texttt{No assumption}, the issue lies in the lemma premises or the local context. \\
\midrule
6 & Expand ``by'' patterns & Rewrite compressed forms such as \texttt{by rewrite}, \texttt{by apply:}, \texttt{have \dots by \dots}, and \texttt{case \dots; by \dots} into explicit proof scripts. This exposes the exact step that fails or the exact branch that remains open. After expanding one \texttt{by} boundary, repair that boundary only. Do not start guessing alternative tactics before reading the first real error, and compress back into \texttt{by} only after the expanded script closes reliably. \\
\midrule
7 & Syntax-driven rewrite & Before every rewrite, check whether the left-hand side of the intended lemma is literally a subterm of the current goal. If it is not, add a bridge step first instead of rewriting from mathematical intuition alone. \\
\midrule
8 & Local bridge lemmas & Use a small local bridge lemma when the mismatch is specific to the current branch or to a fixed local expression. Extract a generic lemma only when the same normalization gap recurs across proofs. \\
\midrule
9 & Big-op normalization order & Normalize inner constant sums or boolean-valued sums first, then perform outer distribution, and only  use multiplication-oriented rewrites afterward. Keep the branch in one stable normal form rather than bouncing among big operators, \texttt{iter}, and multiplication. \\
\midrule
10 & Failure signatures & Failures of \texttt{mul1n}, \texttt{mulnC}, or \texttt{big\_ord\_recr} usually indicate that the goal has not yet reached the required syntactic shape. Once the branch is clearly about \texttt{count}, \texttt{sum1\_count}, or \texttt{Nat.min}, it should be handled by the count-bridging skill instead. \\

\midrule
12 & Error priority \& subgoals & Fix syntax and typing errors before addressing tactic failures. Whenever a proof has multiple subgoals, manage them explicitly with bullets or braces instead of letting the proof drift structurally. \\
\midrule
13 & Tactic selection & Choose tactics from cheaper to more specialized ones, such as \texttt{reflexivity}, \texttt{lia}, \texttt{ring}, \texttt{tauto}, \texttt{congruence}, \texttt{auto}/\texttt{eauto}, and \texttt{decide}/\texttt{native\_decide}. For composite goals, decompose the goal first and automate each component separately. \\
\midrule
14 & Rewrite discipline & When dependent rewriting becomes ill-typed, prefer moves such as \texttt{generalize dependent} or \texttt{subst}. Use \texttt{assert}, \texttt{pose proof}, and \texttt{set} to name intermediate facts instead of hiding too much work inside long inline tactic chains. \\
\midrule
15 & Cleanup \& final check & After a proof compiles, clean it up, choose deliberately between \texttt{Qed} and \texttt{Defined}, follow the intended import and Ltac2 conventions, and run an actual compilation check such as \texttt{coqc}. A proof is not complete until temporary holes such as \texttt{admit} or \texttt{Admitted.} have been removed. \\
\bottomrule
\end{tabular}
\end{table*}



To solve this immediate obstacle, we created a proving skill for situations where lemma application fails to expose subgoals. The key idea is to distinguish between two kinds of premises: postponable premises, which should naturally appear as subgoals after apply or eapply, and early-bound arguments, which must be fixed before the theorem can be correctly instantiated. The procedure is deliberately minimal. First, the agent tries a goal-driven application. If Coq shows normal subgoals, all obligations are treated as postponable and left to normal proof search. If Coq instead reports unresolved existential variables or a failed instance construction before any meaningful subgoal appears, the agent inspects the theorem’s interface, finds the earliest argument that cannot be inferred, and supplies only that value before retrying.

Crucially, the skill forbids falling back to fully explicit proof terms like exact (@lemma ...). Such terms hide the obligation structure and force the agent to manually reconstruct binder order and instance placement, which harms robustness. By only providing the minimal missing binder, the skill preserves the locality and reliability of theorem application, turning the invisible precondition chain into a list of ordinary subgoals that can then be attacked with other proving techniques.



We observe that, when proving difficult lemmas with long proofs, it is challenging for an LLM to prove a lemma end-to-end. It is far more effective to first decompose the lemma into smaller subgoals, each with a much shorter proof than the original. This also aligns with how humans approach complex lemmas: divide and conquer. One might ask why not use a single agent type that can adaptively decide whether to decompose a lemma or prove it directly. Our observation is that, when given the option to decompose, the agent tends to favor this option when facing difficult goals, rather than attempting to prove them directly. Figure \ref{} shows an example where the LLM decomposes a lemma in a meaningless way that does not advance the proof. This pattern recurses, causing all agents to perform shallow decompositions and offload the real work, with no one actually solving anything.
Even strict prompt instructions discouraging premature decomposition prove ineffective. The core issue: we want the LLM to try its best before decomposing, but there is no quantitative standard for the LLM to judge whether it has "tried its best." Thus, we introduce external control with clear quantitative limits. While not optimal, this approach is far more effective than relying on the LLM's self-assessment.


\rtc{
The subagent prompt is constructed as a layered, session-local bundle. For each unresolved proof region, a child session is launched with the target file, enclosing theorem, local goal, replacement contract, frozen region text, editable boundaries, and metadata. Each turn then adds the current proof-state snapshot, including the focused goal and relevant hypotheses. Thus, the subagent does not inherit the prover’s full context, but receives sufficient structured context to respect its ownership boundary and perform interactive proof search within the assigned region.
}

\rtc{
When dispatching a subtask, the system does not forward the original prompt for P-Agent. Instead, it rebuild the child prompt through a staged construction pipeline. Starting from the parent-provided subtask prompt, the task tool checks whether the target worker is a D-Agent. If so, it prepends a structured assignment block that explicitly specifies the local proof obligation, including the assigned context, editable proof region, subgoal contract, and local skeleton. The system then injects a block that encodes execution-time constraints, such as recursion depth limits, split budget, strict prefix-order editing of proof holes, and escalation conditions. Only after these lemma-specific control layers have been added does the system resolve inline prompt references into structured prompt parts, such as file references and agent references. This design ensures that a D-Agent receives not only the parent's high-level intent, but also an explicit statement of ownership and a runtime policy that constrains how the local proof obligation may be solved.
}


\paragraph{Goal Focus Discipline.}
This skill addresses proof-state drift caused by structural tactics such as \texttt{case}, \texttt{destruct}, \texttt{split}, \texttt{apply/negP}, and \texttt{have}. Its central observation is that many Coq failures are not caused by missing mathematical facts, but by a mismatch between the visible script and the actual number of live goals. Accordingly, the skill requires the agent to inspect the current goal count after every tactic that may split, close, or redirect the proof. When more than one goal is open, the skill switches the agent into a structural recovery mode: branches must be managed with bullets, local lemmas introduced by \texttt{have} must be proved inside braces before returning to the outer proof, hidden wrappers must be unfolded before case-splitting on boolean heads, and apparently finished branches must be closed explicitly. This makes the skill particularly effective for errors such as ``Expected a single focused goal but 2 goals are focused,'' where downstream tactic failures are often only secondary symptoms.











We develop proving skills to enhance the subagent's capability of proving their delegated subgoals. The proving skills are generated in a semi-automated way with the help of LLM. 
Concretely, we do it in this way.
we select $60$ lemmas from Prosa (a small fraction of the Prosa lemmas) as \emph{training lemmas}. The selection criteria are as follows. First, we choose lemmas whose proofs span different tactic counts (i.e., lemmas of varying difficulty). Second, we sample lemmas from different files and, whenever possible, different subdirectories within Prosa to maximize diversity.


We use a preliminary version of \ours\ (already adding the external tools and the Prosa library) to prove these lemmas, and collect the traces of the proving procedure. Then we send these traces to LLM to let the LLM to analyze the failure reason and to generate skills to solve these problems. More specifically, we first use LLM to divide each trace into segments, each doing a local task, for example, fixing a particular error or generating a proof for a subgoal, for example, fixing a particular error or generating a proof for a subgoal. \guan{the segement iterate and finally succeed?} We send the segments to LLM one by one to generate proving skills. For each segment, we prompt the LLM to analyze what problem is being solved in this segment, analyze the cause of this problem, and finally generate a skill to avoid this problem to happen or solve the problem. In this way, the LLM generates a pool of skill candidates. Then we send these skill candidates to the LLM to merge those are addressing the same or similar problems,  ask the LLM to refine the skill according these similar skill candidates to cover their common things. Finally, we manually review the remaining skills candidates, select the $17$ proving skills listed in Table \ref{tab:proving_skill_summary}. 



Due to the space limit, we will not elaborate on each of these proving skills. We will only elaborate the last one, the \textbf{ Goal-driven Lemma Instantiation} skill, which solves a problem specific to our schedulability analysis problem using Prosa.
As explained in Section~\ref{}, Prosa has a carefully designed, highly structured hierarchy that encourages lemma reuse across different task models. To apply a such lemma, its preconditions must be satisfied, and those preconditions themselves depend on further preconditions, eventually reaching the specific assumptions of the task model being used. Applying such lemma in the proof often fails. The problem is that in order to use such a lemma, we must provide all these preconditions and extra parameters correctly. 
When the proving agent tries to apply such a lemma, it tries figure out what to be sent exactly for these preconditions and parameters. If any precondition is incorrect, then applying this lemma will lead to a error. For example, in the Prosa, the 
\[
\scriptsize
\texttt{uniprocessor\_response\_time\_bound\_restricted\_supply\_seq}
\]
lemma has \guan{??} preconditions and \guan{??} parameters to be filled in. In order to apply this lemma with all these precondition, the proof needs to be written like in Figure \ref{???}. This is very difficult for the agent to write correctly, and we observe that when encounter such situation in the proof, the proving agent will struggle with finding all the correct parameters. The agent will just repeat to guess these parameters, send to the external Coq tools  and get error message and try to guess again, and in most cases it will never succeed to figure out all the parameters. 
Giving the trace to the LLM to generate proving skills to solve this problem does not work because the LLM simply does not know how to solve this problem. However, there is actually a very simple solution to this problem: besides of using (@lemma ...) to apply this lemma with all parameters, Coq also allows to use  (apply ...), with this lemma, and then 
all these preconditions and parameters become explicit goals,
and these goals are usually relatively easy to prove, many of them even can be automatically resolved by built-in tactics. For example, for the example in Figure \ref{??} can be easily solved by the proof script in Figure \ref{}, where line 1 apply the lemma without providing the preconditions and parameters, 
which will lead to a number of goals to be resolved, and then simply using the tactics \guan{try done}, all these goals are automatically resolved. 



In the following we discuss why the above approach using LLM to analyze the traces of proving lemmas is able to generate useful proving skills. For the proving skill, the trace contains more useful information for the LLM. In the traces, usually the agent iteratively try to solve a local problem, which 
has a very clear standard of being success or failure. The LLM can see in the trace, how it fails again and again, and can see the feedback information, including the error message and current proof states, and eventually how the problem is solved after many iterations. By looking at the success and failure attempt, the LLM have strong information to see what's doing wrong in the failed attempt. The key is that as the LLM can iterative many times, it still may produce a success attempt even if it fundementally does not know how to solve this problem. By comparing the correct attempts and the incorrect attempts, the extracted proving skill indeed provide some extra knowledge the  LLM originally does not know.

Note that the proving skills for subagents we discuss here and the decomposition guideline we introduced in Section \ref{subsec:lemma_decomposition} are fundamentally the same: adding extra information into the prompt of the LLM to enhance it capability of solving problems. However, the way they are obtained are different. The decomposition guideline are developed by human expert manually, while the develop skills are developed by using LLM to analyze the proof traces plus certain human intervention.
Actually, we also tried to use the similar way as generating proving skills to leverage the proof traces and LLM to extract useful decomposition guideline, however it turns out the result is very bad, there is no useful decomposition generated in this way. We conjecture that the reason is that the impact of decomposition is not local and is vague. The LLM struggles to understand from what will happened later to analyze why the decomposition is insufficient, and how to do refined decomposition. Therefore, in this work, we still rely on manual effort to provide the decomposition guidance.

Besides the way they are obtained, the way they are used are also different. 
When using them, we put the decomposition guideline directly into the prompts to the agent, i.e., the agent sees these principles all the time, but for proving skills, we put them into the skill files and the agent will load them on demand: by reading its abstract description, only if the agent feels this skill is useful, it will load this skill. Moreover, the number of skills are larger and many skills are only needed under specific situations. By this design, we manage to let each subagent to have a shorter context. This is especially because we expect for \ours\ to be used by other researchers, everybody can develop more and more proving skills. Currently we put the decomposition guideline directly into the prompts to the primary agent merely because the number is still very small and all of them are commonly used, so the benefit of making them into load-on-demand skill files is not significant. However, this totally does not prevent users to develop their own decomposition guidance as load-on-demand skill files.



\subsection{Agentic Systems and Agent Skills}
\guan{do not touch this part}
Recent LLM-based systems increasingly move beyond single-turn generation toward agentic architectures, where an LLM interacts with tools, memory, feedback, and external environments over multiple steps. A useful distinction is between workflow-based systems and autonomous agents. Workflow-based systems orchestrate LLM calls and tools through predefined control paths, such as prompt chains, routing, evaluator--optimizer loops, or fixed tool pipelines. Autonomous agents, by contrast, dynamically decide which actions to take, which tools to call, what intermediate information to retain, and when to revise their plans according to environmental feedback. Representative methods reflect this shift: ReAct \cite{react} interleaves reasoning traces with task-specific actions, Toolformer \cite{toolformer} studies how language models can learn to invoke external APIs, Reflexion \cite{reflexion} improves agents through verbal feedback stored in memory, and AutoGen \cite{autogen} provides a framework for constructing multi-agent systems through configurable conversations among LLM agents, tools, and humans.

In interactive theorem proving, agentic systems instantiate these components as proof-state observation, premise retrieval, tactic execution, proof checking, failure analysis, and iterative repair. RocqStar \cite{rocqstar} combines similarity-driven premise retrieval with a multi-stage agentic pipeline for Rocq generation, using planning, multi-agent debate, and reflection to improve proof success. ReCent-Prover \cite{recentprover} further emphasizes reasoning-centric proof automation by conditioning retrieval on LLM-generated proof plans rather than only subgoal similarity, and by using reflection to evaluate failed proof attempts before retrying. These systems show that proof automation is moving from one-shot tactic generation toward agents that plan, retrieve, execute, observe proof-state feedback, and revise their strategies.

Agent skills provide a complementary mechanism for making such agents more specialized and reusable. Rather than treating every task as a fresh prompt, a skill encapsulates reusable procedural knowledge, such as a tool-use pattern, a domain-specific routine, a verified code fragment, or a strategy that can be retrieved and composed in future tasks. Voyager \cite{voyager} makes this idea explicit through an ever-growing library of executable skills, where complex behaviors are stored, retrieved, and reused to solve new tasks. More broadly, agent skills can be implemented as callable tools, prompt modules, memory entries, code snippets, or higher-level procedures. In proof automation, however, this idea remains less developed: existing systems mainly retrieve premises, previous proofs, proof plans, or failed-attempt summaries, but they rarely represent reusable proof procedures as explicit skills with domain-specific preconditions, effects, and adaptation rules. A broader survey of LLM-based theorem proving is available in \cite{llm_atp_survey}.

Overall, this body of work shows a clear shift in proof automation from isolated tactic prediction toward systems that combine proof synthesis, retrieval, compiler feedback, iterative repair, and agentic control. These systems make proof search more flexible than earlier tactic- or solver-based automation: they can generate longer proof fragments, exploit local context, revise failed attempts, and sometimes incorporate informal explanations or proof sketches as auxiliary guidance. However, in specialized verification domains such as real-time scheduling, successful proofs often depend on recurring semantic structures: scheduling assumptions, workload and processor models, invariants, response-time bounds, rewriting conventions, and lemma sequences that apply only under particular conditions. Existing methods still largely treat reusable knowledge as retrieved premises, similar proofs, or short-term proof-state context, rather than as domain-specific proof procedures. Current retrieval and agentic mechanisms do not yet make these procedures explicit as reusable skills with applicability conditions, required assumptions, expected effects, and adaptation strategies. This leaves a gap between general LLM-based proof generation and domain-aware proof automation for Coq/Rocq developments built around specialized verification libraries.



% \subsection{Autoformalization}

% Pre-LLM Coq automation largely operates after a goal has been formalized: tactics, solvers, and proof-search tools try to discharge obligations that already exist inside the proof assistant. Autoformalization addresses a complementary problem: translating informal mathematical or specification-level content into machine-checkable formal artifacts. Its inputs may include theorem statements, requirements, proof outlines, or natural-language proofs, and its outputs may range from definitions and theorem statements to proof sketches or full proof scripts. This task has been studied through controlled languages, corpus-based translation, symbolic disambiguation, semantic parsing, neural translation, and, more recently, LLM-based methods.


% Early autoformalization work focused on connecting informal mathematical text with formal libraries and proof assistants without relying on large language models. Kaliszyk et al. \cite{informal_formal_translation} proposed corpus-based translation methods between informal and formal mathematics, framing autoformalization as a data-driven alignment problem between mathematical prose and formal corpora. Wang et al. \cite{neural_informal_formal} later explored neural translation from informal to formal mathematics, showing that sequence models could learn nontrivial mappings from mathematical text to formal expressions. M{\"u}ller and Kaliszyk \cite{symbolic_disambiguation} further studied the disambiguation of symbolic expressions in informal documents, addressing a key obstacle for formalization: informal mathematical notation is often underspecified and must be resolved before it can be translated into a formal language. These works establish autoformalization as a broader research problem that predates the current LLM-based setting. 

% Recent LLM-based work has expanded autoformalization across multiple target systems and application settings. For Coq/Rocq, directly relevant LLM-based work remains limited, but multi-language formalization efforts have begun to include Coq as a target system. Cao et al. \cite{informal_to_formal_requirements} construct instruction-style data for translating natural-language requirements into verifiable formal artifacts across Coq, Lean4, Dafny, ACSL, and TLA+, providing a formal-verification-oriented benchmark for LLM-based informal-to-formal translation. Beyond Coq/Rocq, Wu et al. \cite{autoformalization_llm} showed that LLMs can translate natural-language mathematical problems into formal specifications and use the resulting data to improve downstream theorem proving. ProofNet \cite{proofnet} pairs informal mathematical statements and proofs with formal theorem statements to evaluate faithful autoformalization. Draft, Sketch, and Prove \cite{draftsketch} translates informal proofs into formal proof sketches that guide proof search. RAutoformalizer \cite{rautoformalizer} emphasizes retrieving the right formal dependencies to avoid plausible but ill-formed formalizations. 
% Survey \cite{autoformalization_survey} summarizes datasets, target systems, evaluation methods, and application domains across this line of work.

% Autoformalization is adjacent to proof generation, but it differs in emphasis. Autoformalization centers on translating informal content into formal artifacts, so informal statements, specifications, or proofs are part of the task itself. Proof generation may use informal explanations or paper proofs when available, but it can also start from an already formalized theorem statement and construct a checker-accepted proof script from the formal goal, library context, and prover feedback. Thus, informal text is not a mandatory input for proof generation, which is the focus of the Coq/Rocq systems reviewed below.

% \subsection{LLM-based Autonomous Theorem Proving}
% \begin{itemize}
%     \item general ATP (including lean and others, how LLM-based ATP achieves impressive results)

%     \item specific to Coq/Rocq
% \end{itemize}

% Given a formal theorem statement, recent work has begun to use LLMs as proof-producing components for interactive theorem provers. This direction has been explored across several formal systems, from early generative neural provers for Metamath and Lean-style benchmarks~\cite{gptf,htps}, to retrieval-augmented and model-training approaches for Lean~\cite{leandojo,llemma,deepseekprover,leanstar,deepseekproverv2,kiminaprover}, and to Isabelle/HOL systems that combine language models with hammer-style automation or proof repair~\cite{thor,baldur}. Due to space constraints, we focus below on Coq/Rocq systems, which are most closely related to our evaluation setting.

% This setting is distinct from autoformalization: rather than translating informal mathematical content into formal statements or proof sketches, these systems assume that the theorem has already been formalized and address the subsequent task of constructing a machine-checkable proof. Compared with earlier tactic-based or solver-based automation, LLM-based systems can synthesize longer proof fragments, make use of intermediate proof-state information, and revise failed attempts based on compiler feedback. CoqPilot \cite{coqpilot} packages this capability as a Coq-oriented development assistant, generating candidate proofs inside the proof-engineering workflow. COPRA \cite{copra} formulates proof search as an in-context interactive process, where the model proposes tactics, observes proof-state feedback, and continues the proof through a dialogue with the prover. PALM \cite{palm} further shows that proof generation can be strengthened by a generate-then-repair architecture, where low-level proof errors produced by the model are analyzed and repaired using symbolic procedures. Together, these systems demonstrate that LLMs can act as practical proof-generation components for Coq-style environments, while remaining complementary to autoformalization methods that operate before the theorem-proving stage.

% More recent systems further combine proof generation with retrieval and multi-step
% interaction. Rango \cite{rango} retrieves relevant premises and similar proofs from the
% current Coq project at each proof step, showing that project-local retrieval can
% substantially improve proof synthesis. RocqStar \cite{rocqstar} and ReCent-Prover \cite{recentprover}
% extend this trend toward agentic proof automation, introducing planning,
% reflection, and strategy-aware retrieval into Rocq proof generation.


% \begin{table}[t]
% \centering
% \tiny
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{Representative LLM-based theorem proving systems for Coq/Rocq. ``Avail.'' means the paper/tool is publicly available; ``Open'' means the implementation is open-source.}
% \label{tab:llm_proof_automation}
% \begin{tabular}{@{}lclccp{4.5cm}@{}}
% \hline
% Work & Year & Prover & Avail. & Open & Retrieval? \\
% \hline
% CoqPilot~\cite{coqpilot}
% & 2024 & Coq & Yes & Yes
% & Context theorem selection from completed proofs; Jaccard/distance ranker, non-RAG \\

% PALM~\cite{palm}
% & 2024 & Coq & Yes & No
% &  BM25 premise retrieval over project environment; retrieved premises/defs are appended to the prompt \\

% Rango~\cite{rango}
% & 2025 & Coq & Yes & No
% & Adaptive RAG at each proof step; retrieves relevant premises and similar proofs from the current project \\

% COPRA~\cite{copra}
% & 2023 & Coq & Yes & No
% & External lemma retrieval; retrieved lemmas are included with search history in the prompt \\

% RocqStar~\cite{rocqstar}
% & 2025 & Rocq & Yes & Yes
% & Similarity-driven premise retrieval; self-attentive embedder for premise selection \\

% ReCent-Prover~\cite{recentprover}
% & 2026 & Rocq & Yes & No
% & Planning-conditioned retrieval; retrieves lemmas/proofs according to LLM-generated proof plans rather than subgoal similarity \\
% \hline
% \end{tabular}
% \end{table}



% \subsection{Pre-LLM Theorem Proving Automation}

% Before the rise of LLM-based theorem proving, Coq/Rocq had already accumulated a rich ecosystem of automation techniques for reducing manual proof effort. At the most immediate level, Coq provides tactic-level automation for routine proof obligations. General-purpose tactics such as \texttt{auto}, \texttt{eauto}, \texttt{intuition}, \texttt{firstorder}, and \texttt{congruence} search through hypotheses and hint databases, while domain-specific procedures such as \texttt{omega}, \texttt{lia}, \texttt{nia}, \texttt{micromega}, \texttt{ring}, and \texttt{field} automate arithmetic and algebraic reasoning. These tactics are indispensable in large developments, but their scope is mostly local: they solve isolated subgoals once the surrounding proof structure has already been supplied by the user.

% Building on Coq's computational foundation, another major line of work developed proof by reflection. SSReflect \cite{ssreflect} and Mathematical  Components \cite{mathcomp} use boolean reflection, structured rewriting, canonical structures, and algebraic hierarchies to make recurring proof patterns reusable and efficient. CoqEAL \cite{coqeal} further explored how efficient computational algorithms can be connected to proof-oriented specifications. This reflective style is powerful because computation remains within Coq's trusted logic, but it requires substantial proof-engineering effort, including reification procedures, verified decision procedures, and reflection-friendly library design.

% Coq automation was also extended by connecting the proof assistant to external automated reasoning tools. SMTCoq \cite{smtcoq} and smt4coq \cite{smt4coq} translate Coq goals to SMT solvers such as Z3 or CVC-style engines and reconstruct or check solver certificates inside Coq. CoqHammer \cite{coqhammer} brings hammer-style automation to Coq by combining premise selection, translation to first-order logic, ATP calls, and proof reconstruction. These tools substantially expand the reach of automation for first-order, equality, arithmetic, and SMT-supported reasoning. However, they remain sensitive to translation quality, premise selection, and reconstruction failures, especially when proofs involve dependent types, higher-order structure, complex induction, or domain-specific invariants.

% Alongside solver integration, Coq users and tool builders developed increasingly expressive ways to program automation directly inside the proof assistant. Ltac \cite{ltac} and its successors or alternatives, including Ltac2, Mtac/Mtac2 \cite{mtac,mtac2}, Coq-Elpi \cite{coqelpi}, and MetaCoq \cite{metacoq}, provide mechanisms for building domain-specific tactics, inspecting proof states, and manipulating Coq terms and proof terms. These systems made it possible to encode reusable proof strategies for mature verification projects, but they also shifted part of the burden from individual proof scripts to the engineering of proof infrastructure.

% Prior to LLMs, researchers further explored machine-learning guidance for Coq proof automation. ML4PG \cite{ml4pg} used learning techniques to identify similar proof patterns in Coq/SSReflect developments, while CoqGym \cite{coqgym} provided a large-scale dataset and environment for learning tactic prediction from real Coq proofs.
% Systems such as Tactician \cite{tactician}, Proverbot9001 \cite{proverbot9001}, and TacTok \cite{tactok}, as well as CoqGym neural baselines such as ASTactic \cite{coqgym}, investigated learned tactic prediction, local proof search, and semantics-aware proof synthesis. These approaches improved tactic ranking and proof-step suggestion, but they largely remained tied to local proof states and existing tactic interfaces.

% Taken together, pre-LLM Coq automation significantly reduced the burden of routine reasoning through tactics, reflection, SMT/ATP integration, metaprogramming, and learning-guided search. Yet these techniques did not fully close the gap between local proof automation and high-level proof engineering. Tasks such as decomposing large verification goals, inventing reusable lemmas, selecting abstractions, coordinating induction arguments, and maintaining proofs across evolving formal developments still largely depended on expert human guidance.



\begin{table}[t]
\centering
\tiny
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{0.95}
\caption{Representative LLM-based Coq/Rocq theorem proving systems. ``Avail.'' denotes practical usability; ``Source'' denotes public source availability. \guan{change}}
\label{tab:llm_proof_automation}
\begin{tabular}{@{}lclccp{4.5cm}@{}}
\toprule
Work & Year & Prover & Avail. & Source & Retrieval? \\
\midrule
CoqPilot~\cite{coqpilot}
& 2024 & Coq & Yes & Yes
& Context theorem selection from completed proofs; Jaccard/distance ranker, non-RAG \\

PALM~\cite{palm}
& 2024 & Coq & Yes & Yes
& BM25 premise retrieval over project environment; retrieved premises/defs are appended to the prompt \\

COPRA~\cite{copra}
& 2024 & Coq & Yes & Yes
& External lemma retrieval; retrieved lemmas are included with search history in the prompt \\

RocqStar~\cite{rocqstar}
& 2025 & Rocq & Yes & Yes
& Similarity-driven premise retrieval; self-attentive embedder for premise selection \\

Rango~\cite{rango}
& 2025 & Coq & No$^{*}$ & Yes
& Adaptive RAG at each proof step; retrieves relevant premises and similar proofs from the current project \\

ReCent-Prover~\cite{recentprover}
& 2026 & Rocq & No & No
& Planning-conditioned retrieval; retrieves lemmas/proofs according to LLM-generated proof plans rather than subgoal similarity \\
\bottomrule
\end{tabular}
\end{table}
%\subsection{LLM-based Autonomous Theorem Proving}


\begin{itemize}
  \item \textbf{Native tools} \guan{how should we catgarize the native tools? all of them all command lines? or some are not?}
  \begin{itemize}
    \item \texttt{bash}: Executes shell commands inside the workspace for tasks such as build, test, and git operations.
    \item \texttt{batch}: Runs multiple registered tool calls in parallel to reduce interaction overhead.
    \item \texttt{codesearch}: Queries an external code/documentation search service for API, library, and SDK context.
    \item \texttt{glob}: Finds files by glob patterns for fast path-level discovery.
    \item \texttt{grep}: Searches file contents by regular expression for symbols, config keys, or text snippets.
    \item \texttt{list}: Prints a directory tree view to quickly inspect workspace structure.
    \item \texttt{read}: Reads files or directories, and can also pass image/PDF content to the LLM as attachments.
    \item \texttt{edit}: Performs a localized string replacement in one file and returns diff-aware feedback.
    \item \texttt{multiedit}: Applies multiple localized edits to the same file in sequence.
    \item \texttt{apply\_patch}: Applies structured patches for multi-file add/update/delete/move changes.
    \item \texttt{todowrite}: Updates the current session's todo list for multi-step task tracking.
    \item \texttt{todoread}: Reads the current session's todo list for state recovery and progress inspection.
  \end{itemize}


  

\section{Some points to remember}\label{methodology}

\guan{
2026-03-25

\begin{itemize}
\item developed tools
\begin{itemize}
\item coqc: a filter: opencode link coq compiler: opencode generated code sent to coq compiler, return success or failure (or error). reference anything: no? we can claim, we have to write it by ourself. we are the first one doing this?  return only error message and line number. filter.
opencode can use terminal tool can do this, but not optimized.
warining/compiling procedure. TODO: to be confirmed by Tianchi.

\item coqtop: 

\item proof-guard: to avoid (1)
the same code generated repeatedly (2) 


x

\item TODO: opencode justify, is there any evaluation about the "capability" comparison opencode, rely on using deepseek prover to defend this.


\end{itemize}
\end{itemize}

}

\guan{how the pdf paper is read?}

In this section, we detail the key components and processes involved in our approach.
We begin by describing the enhancements made to the PROSA benchmark to facilitate LLM-based proof generation.
Next, we discuss the integration of domain-specific knowledge related to real-time systems.
Finally, we present the dynamic agentic workflow designed to enable dynamic proof strategy generation
using LLMs.

\subsection{Agent for Formal Proof Generartion}



% \subsection{Integrating Domain-Specific Knowledge of Real-Time Systems}
% To enhance the capability of LLMs in generating formal proofs specific to real-time systems,
% we integrate a domain knowledge plugin into the Rocpilot system. This plugin provides access 
% to a curated knowledge base of real-time systems concepts, theorems and proof strategies.

% \subsection{Agentic Workflow for PROSA-based Proof Generation}







\subsection{Other Implementation Issues}




\guan{TIANCHI: WRITE HERE}

\rtc{
Sandbox for cheat avoidance(auto build sandbox env for proof), mechanical check on edit violation.


}




\begin{table}[htbp]
\centering
\caption{Skill grouping and trigger conditions}
\label{tab:skill-groups}
\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{
    >{\centering\arraybackslash}p{0.05\columnwidth}
    >{\centering\arraybackslash}p{0.07\columnwidth}
    >{\raggedright\arraybackslash}p{0.77\columnwidth}
}
\toprule
\multicolumn{1}{c}{\textbf{group}} &
\multicolumn{1}{c}{\textbf{skills}} &
\multicolumn{1}{c}{\textbf{trigger condition}} \\
\midrule
1 & 1--4 &
Use this skill when a proof branch is drifting among indicator sums,
filtered big operators, counts, and min-based bounds, and the immediate
need is to normalize the expression into a stable counting form before
finishing the arithmetic. \\
\midrule
2 & 5--6 &
Use this skill when Rocq reports a failure on a compressed
\texttt{by \ldots} script and you need to expand it to reveal the first
concrete error, missing premise, or extra subgoal. \\
\midrule
3 & 7--10 &
Use this skill when a rewrite seems mathematically correct but fails
because the current goal is in the wrong syntactic shape, especially
across big operators, iter, addition, or multiplication. \\
\midrule
4 & 11--15 &
Use this skill as the default fallback when a Rocq proof needs general
structure, error-handling discipline, and step-by-step proof management. \\
\bottomrule
\end{tabular}
\end{table}
\guan{junyi: list the automated generated skill points here}





\guan{organizing the proving skills into skill files}

\textbf{Scope of Modification}: The sub-agent's edit access is strictly limited to its assigned proof-region. Any text outside this designated region must be treated as read-only, explicitly prohibiting the sub-agent from altering external proof scripts.


\guan{the timeout threshold}

\guan{add our design about prevent cheating ... }


\guan{\textbf{General Prompt}}. The proof starts with a general prompt

\guan{how the different agent interact with each other?}

\guan{prevent cheating? verifier}

\guan{context compaction} The memory management takes charge of compacting the context of a working agent from time to time, and distill useful proving skills and 
store them into the proving skill set.

When the agent is working, it will iteratively generate output tokens and these output tokens, together with the information obtained from using the external tools, will be appended to the query of the last round, to be used as the query in next round, as shown in the Example in Figure \ref{}. Therefore, the query length keeps growing as the iteration goes on, 
and will eventually exceed the allowed context length of the backbone LLM. Even if not exceeding the context length limitation, a long context
may be bad for the inference because it may affect the attention (\guan{what is the terminology?}). Therefore, the memory manager will trigger a context compaction when the context length of the agent reaches a certain threshold. The context compaction will send the context context to the LLM, and let it output the compacted context containing the following parts:
\guan{need to say what extra we put: the system prompt is put into it again}
\begin{itemize}
\item xxx
\item xxx
\item xxx
\item Experience. The experience gained so far. 
\end{itemize}

\guan{can move this discussion to the experiment}
Setting a good context compaction trigger threshold is important to the performance. If the threshold is too high, then the context compaction is lazy. This may be bad for the inference quality cause the long context may make the attention weaker, making the not pay sufficiently attention to the content in its context. (\guan{For example, ???}).
Moreover, when the context is overly lengthy, the inference efficiency will degrade. Note that the linear expansion way of increasing the context length is friendly to KV cache. Therefore, it has a good chance that every iteration the query tokens that stay the same as the last round will be hit on KV cache, which is much more efficient than computing the KV values for all the tokens from scratch. However, a very long context may still be inefficient even if with KV cache hit, since 
the attention between the new tokens with all the tokens in the past context still need to compute, which is a huge effort when the context is very long. The 




\subsection{Context Compaction and KV cache performance}

\guan{write it later}

\ljy{

The original theorem is stated as follows.
\begin{theorem}[Schedulability Condition]
\label{thm:schedulability-condition}
The task set is schedulable if and only if, for each task \(\tau_k\), one of the following conditions holds:
\begin{enumerate}
    \item
    \[
        \sum_{i \neq k} \min \left( \overline{I}_{i,k}, D_k - C_k \right)
        < m \left( D_k - C_k \right).
    \]

    \item
    \[
        \sum_{i \neq k} \min \left( \overline{I}_{i,k}, D_k - C_k \right)
        = m \left( D_k - C_k \right)
    \]
    and
    \[
        \exists h \neq k : 0 < \overline{I}_{h,k} \leq D_k - C_k .
    \]
\end{enumerate}
\end{theorem}

During the formalization of this theorem, Case~3 revealed a missing assumption in the original statement. 
The agent produced a counterexample showing that Theorem~\ref{thm:schedulability-condition} requires the stronger condition \(C_k < D_k\), rather than the standard assumption \(C_k \leq D_k\). 
If \(C_k = D_k\), then \(D_k - C_k = 0\). 
As a result, the first alternative reduces to the impossible goal \(0 < 0\), and the second alternative requires
\[
    0 < \overline{I}_{h,k} \leq 0,
\]
which is contradictory. 
Therefore, the theorem is not sound unless the boundary case \(C_k = D_k\) is ruled out.

This issue is not explicitly addressed in the paper. 
It is especially easy to overlook because the conventional sporadic-task model in real-time scheduling assumes \(C_k \leq D_k\), and PROSA's \texttt{is\_valid\_sporadic\_task} predicate adopts the same non-strict condition. 
Hence, the formal proof requires an additional assumption \(C_k < D_k\) to precisely capture the intended theorem.
}



\guan{remove human hint}
\textbf{PB-w/o-H}. This variant removes the human-written proof hints from \ours, i.e., it does not read the content of the corresponding research paper. PB-w/o-H proves 15 lemmas, only slightly fewer than \ours. This indicates that the formal context in Prosa already provides strong guidance for many lemmas, and that \ours\ can often infer the proof direction from definitions, existing lemmas, and proof states. The token numbers show that hints are not always necessary: for several solved lemmas, PB-w/o-H succeeds with comparable or fewer tokens than \ours. However, hints still help on difficult cases where the search space is large. Thus, natural-language hints are useful high-level guidance, but they are not the dominant source of performance.



  PB-w/o-H & \makecell{\ding{52} \\ 36,340} & $\infty$ & $\infty$ & \makecell{\ding{52} \\ 11,238} & \makecell{\ding{52} \\ 358} & \makecell{\ding{52} \\ 3,501} & \makecell{\ding{52} \\ 1,257}& 
  \makecell{\ding{52} \\ 16,550}& 
  \makecell{\ding{52} \\ 41,562} & \makecell{\ding{52} \\ 1,398} & \makecell{\ding{52} \\ 1,321} & \makecell{\ding{52} \\ 31,716} & \makecell{\ding{52} \\ 5,096} &
  \makecell{\ding{52} \\ 47,416}& \ding{56} & \ding{56} & \makecell{\ding{52} \\ 23,906} & \ding{56} & \makecell{\ding{52} \\ 1,833} & \ding{56} & \ding{56} & \makecell{\ding{52} \\ 21,157} & \makecell{\ding{52} \\ 177} or \ding{56} & \makecell{\ding{52} \\ 9,278} & 16\color{red}17\\



\begin{table}[htbp]
\centering
\caption{Source of Case Study}
\label{tab:source_of_case_study_notprosa}
% ccccc 代表5列，每列内容居中对齐 (可按需改为 l 靠左, r 靠右)
\begin{tabular}{ccccc}
\toprule
\textbf{index} & \textbf{pape} & \textbf{Theorem} & \textbf{dependency} & \textbf{} \\
\midrule
1  & \cite{bertogna2005} & Lemma 3 & null &  \\
2  & \cite{bertogna2005} & Lemma 4 & case1 &  \\
3  & \cite{bertogna2005} & Theorem 6  & case1,2 &  \\
4  & \cite{bertogna2007} & Theorem 1& null &  \\
5  & \cite{bertogna2007} & Theorem 2 & null &  \\
6  & \cite{bertogna2007} & Theorem 3 & case3 &  \\
7  & \cite{bertogna2007} & Theorem 4 & null &  \\
8  & \cite{guan2009}& ? & null &  \\
9  & \cite{guan2009} & Lemma 1 & null &  \\
10 & \cite{guan2009} & Theorem 1? & case 8 &  \\
11 & \cite{guan2009} & Theorem 1 & case 17 &  \\
12 & \cite{guan2009} & Lemma 1&  null  \\
13 & \cite{guan2009} & Theorem 2 & case 18 &  \\
14 & \cite{guan2009} & Lemma 2 & case9,12 &  \\
15 & \cite{guan2009} & Lemma 2 & case9,12  &  \\
16 & \cite{guan2009} & Lemma 3  & case14,15 &  \\
17 & \cite{guan2009} & Lemma 4 & case 16 &  \\
18 & \cite{guan2009} & Lemma 5 & null &  \\
19 & \cite{sun2014}& Theorem 3 & case21 &  \\
20 & \cite{sun2014} & Lemma 4  & null &  \\
21 & \cite{sun2014} & Lemma 5 & case20 &  \\
22 & \cite{baruah2015} & Lemma 18.1 & null &  \\
23 & \cite{baruah2015} & Theorem 18.6 & case22 &  \\
24 & \cite{2013ecrts}& Lemma 8 &  null & \\

\bottomrule
\end{tabular}
\end{table}





\subsubsection{Progress Supervisor}

Sometimes the agent may repeat the same actions without advancing the proof, so we developed a \teim{Progress Supervisor} tool to govern the proof development workflow. It consists of two tightly integrated sub-functions: the \emph{Progress Evaluator} and the \emph{Dispatch Governor}.

The primary agent or a subagent invokes the Progress Evaluator after completing a proof region, or whenever it needs to compile the current intermediate version of the target proof. This sub-function performs the following duties:
It launches the Rocq compiler on the current version of the target file, reporting both the overall compilation result and the first compiler error encountered.
It updates the internal states of proof region blocks, creating new compiler certificates for validated regions or invalidating obsolete ones.
It determines whether the latest edit constitutes meaningful proof progress. To make this judgment, it counts all unfinished constructs within the target theorem, including: \texttt{admit} placeholders, empty proof blocks, proofs terminated with \texttt{Admitted} or \texttt{Abort}, theorems that do not yet end with \texttt{Qed}, and the number of proof region blocks that remain unresolved.
Based on this analysis, the Progress Evaluator classifies the outcome into three distinct categories:
\begin{itemize}
\item Hard progress: recorded when Rocq successfully accepts a previously unresolved proof region in its current version, and ProsaBuddy generates a validated compiler certificate for that specific version. 
\item  Structural progress: indicates that an accepted proof decomposition has been written as dependency-complete regions and the resulting proof sketch compiles, yet no new subgoal has actually been proved.
\item  Debug progress: means that the first compiler error now appears later in the proof script (i.e., the error position has moved forward).
\end{itemize}


The Dispatch Governor consumes the records produced by the Progress Evaluator to monitor agent behaviour and enforce scheduling discipline. It actively detects the following patterns of ineffective repetition: consecutive tool calls that yield no hard progress for the same theorem and region, repeated compiler invocations that report the identical first error on unchanged source code, or repeated attempts to dispatch a subagent for that same theorem and proof region.
When the Dispatch Governor identifies that the agent has repeatedly taken actions without advancing the proof, it first reports this as a warning to the LLM. If the same unproductive actions continue, the governor prevents the primary agent from dispatching another subagent for that unchanged theorem and proof region. Superficial modifications—such as changes only to comments, region identifiers, or whitespace, do \emph{not} release this restriction.
If subagent dispatching has been blocked for a specific proof region, the Scheduler may permit a new lemma subagent to be launched only in one of the following two scenarios: (1) The Progress Evaluator has subsequently recorded hard progress for that region, or (2) the primary agent or a theorem-level repair subagent has made a substantive change to the region's Rocq proof commands, target subgoal, or (3) \texttt{depends\_on} declaration, and the modified region has passed the corresponding consistency checks.

\guan{!!!!!!!!!!!!!!!!!}


\ljy{%


ProsaBuddy therefore uses \texttt{checkpoint} to record whether
a previously unfinished proof region has passed Rocq
validation or whether the complete target theorem has passed
Rocq compilation and ends with \texttt{Qed.}. The progress
guard uses these results to detect repeated tool calls or
subagent attempts that neither complete another
proof region nor complete the target theorem. When ProsaBuddy detects that the agent has repeatedly taken
actions without advancing the proof, the progress guard reports
this information to the LLM as a warning. If the same actions
continue without advancing the proof, the progress guard may
prevent the primary
agent from dispatching another subagent
for the unchanged theorem and proof region. This does
not immediately terminate the proof task. Instead, the primary
agent must revise the proof commands, add a required
intermediate lemma, or change the decomposition before another
lemma subagent can be dispatched.
}








\ljy{%


\textbf{Checkpoint and progress guard.}
The primary agent or  subagent calls
\texttt{checkpoint} after completing a proof region,
or when it needs to compile the
current intermediate version of the target proof.
 The tool invokes the Rocq compiler on the
current version of the target file. In addition to reporting
the compilation result and the first compiler error, it updates
the states of the proof region blocks, creates or
invalidates their results, and determines
whether the latest edit constitutes proof progress.

For this purpose, the tool counts unfinished constructs in the
target theorem, including \texttt{admit} placeholders, empty
proof blocks, and proofs terminated by \texttt{Admitted} or
\texttt{Abort}. It also checks whether the theorem ends with
\texttt{Qed} and counts the proof region blocks that
do not have finished.

The tool classifies the result as \emph{hard},
\emph{structural}, or \emph{debug} progress. Hard progress is recorded when Rocq accepts the current version
of a previously unresolved proof region, and
ProsaBuddy records a validation compiler certificate for that version. Structural
progress records that an accepted decomposition has been
written as dependency-complete regions and that the resulting
proof sketch compiles, but it does not claim that any new
subgoal has been proved. Debug progress records the first compiler error occurs later in the proof. Removing a an \texttt{admit} placeholder or an empty proof block without obtaining
a compiler certificate is not classified as hard proof
progress.

The agent runtime uses these progress records to detect
repeated work on the same theorem and proof region.
It records consecutive tool calls without hard progress,
repeated compiler calls that report the same first error for
unchanged source, and repeated subagent
attempts for that theorem and region. After repeated attempts
without hard progress, the runtime first warns the agent and
can subsequently prevent another subagent from being launched
to prove the same theorem and region. Changes only
to comments, region identifiers, or whitespace do not release
this restriction. If the progress guard has blocked further subagent attempts for
a proof region, the Scheduler may dispatch another
lemma subagent only in either of two cases. First,
\texttt{checkpoint} has recorded hard progress. Second, the
primary agent or theorem-level repair subagent has made a
substantive change to the region's Rocq proof commands, target
subgoal, or \texttt{depends\_on} declaration, and the modified
region has passed the corresponding consistency checks.

The progress guard does not establish logical correctness and
does not replace the Checker checks. It controls intermediate
agent actions and can reduce token consumption caused by
repeating subagent attempts that produce neither a new
compiler certificate nor a successful final \texttt{Qed}
check.
}



\ljy{ delete begin}
Our benchmark is constructed from existing papers in the field of real-time scheduling. In the original publications, each theorem or lemma is accompanied by a proof that was manually developed by human.
For \ours\ and OpenCode, we use the relevant portion of the original paper as the human-written proof hint input. Specifically, this input includes the target theorem or lemma itself, its full human-written proof, as well as any supporting definitions, notation, and variables that are referenced within the proof. 
On the other hand, we do not supply such human-written proof hints to PALM, Cobblestone or to RocqStar. The reason is that neither of these three systems exposes an input interface that can read external textual materials. PALM  and Cobblestone operate exclusively through there generate-and-repair workflow, which takes the formal theorem and the current proof state as inputs and iteratively attempts to construct a valid proof. It does not accept additional natural language hints or proof sketches from outside. Similarly, RocqStar is designed around formal Rocq context retrieval; it can query and retrieve relevant formal definitions and theorems from a structured library, but it lacks the ability to ingest free‑text descriptions as external input.
Later in the ablation study we will show that, even if the human-written proof hint is removed, \ours\ still significantly outperforms PALM, Cobblestone and RocqStar. 
\ljy{ delete end}





To ensure that the agent really proves the target lemma rather than bypassing it, we develop a Validator tool for proof integrity checking. 
Validator compares the proof file generated by the agent with the original modeling file to detect whether the agent has changed the problem itself, introduced unproven facts, weakened the theorem statement, or moved the main proof obligation into another global lemma.
{At the beginning of a proof task, Validator records the
\texttt{.v} file containing the target theorem and the original
theorem statement. It also records the source before the
theorem's \texttt{Proof.} command and after its proof
terminator. }

{Before accepting an edit, Validator verifies that the original
theorem statement and all existing imports, definitions,
lemmas, and other global declarations remain unchanged. The
agent may modify the proof commands between \texttt{Proof.} and
the proof terminator. Validator also permits adding imports from
trusted libraries, such as Prosa or MathComp \guan{we allow the official libraries of coq, but now we only choose to include these two, because others do not seem to be useful}, and making
cosmetic changes to comments, whitespace, and formatting.}
\ljy{
\begin{itemize}
\item 
    \texttt{Admitted}, \texttt{admit}, 
    \texttt{Abort},
    \texttt{sorry},
    \texttt{give up}.
    
\item 
\texttt{Axiom}, 
\texttt{Parameter}, \texttt{Parameters}, \texttt{Conjecture}, \texttt{Conjectures}, 
\texttt{Unset Guard Checking},
\texttt{Unset Positivity Checking},
\texttt{Unset Universe Checking},
\texttt{Fail Qed. Abort},
\texttt{Declare ML Module}
\end{itemize}


}

Concretely, it reports cheating if the agent adds constructs such as \texttt{Axiom}, \texttt{Parameter}, \texttt{Parameters}, \texttt{Conjecture}, \texttt{Conjectures}, \texttt{Admitted}, \texttt{admit}, or \texttt{Abort}.
It also detects changes that modify the target lemma statement, change existing model definitions, or introduce new global lemmas or definitions outside the target proof in a way that carries the main proof burden.
These changes are considered cheating because the resulting file may compile without actually proving the original lemma.
On the other hand, Validator allows harmless changes that do not alter the theorem's meaning.
It permits importing additional libraries from trusted sources and making purely cosmetic edits such as comments, blank lines, or formatting changes.
% rtc added begin here
During proof construction,
Validator executes before applying each edit
proposed by an agent to the target file. Before reporting that
the proof task has succeeded, Validator checks
the complete file again. This final check confirms that the target theorem statement and the existing declarations remain
unchanged and that the file contains no forbidden proof
constructs.

For the proof file under test, {Validator compares} the final version with the original proof file to determine whether the agent has attempted to bypass the proof obligation. In our workflow, a lemma is considered successfully proved only when two conditions hold simultaneously.
First, the generated \texttt{.v} file must pass the Rocq compiler check. \ljy{When a generated .v file is successfully compiled, Rocq elaborates the tactic
script into a proof term, and the Rocq kernel checks that this proof term establishes the
declared theorem. Thus, the logical correctness of the generated proof ultimately relies
on the Rocq kernel; the Validator does not replace the kernel.}
Second, the Validator must confirm that the proof does not rely on forbidden edits or semantic changes to the original modeling file.
If either of them fails, the proof attempt is not counted as successful.

Beyond checking the generated proof file itself, we also run each proof task in a file-system sandbox.
{Validator examines the changes made to the target
\texttt{.v} file and permits additional import commands only
for trusted libraries, such as Prosa or MathComp. The
file-system sandbox prevents the agent from modifying the imported library files, project configuration files, or other
Rocq source files.}
The sandbox is an isolated workspace that limits what files the agent can see and modify.
This is necessary because, without such isolation, an agent could bypass the proof task by modifying files outside the intended workspace, such as installed libraries or dependency files.
Such changes could alter the environment in which the theorem is checked, making the proof pass without actually proving the original theorem.




\begin{comment}
    

\begin{itemize}


\item 但是我们发现，让LLM直接生成上面那个incomplete proof，效果非常不好。举例子说明，怎么效果不好（比如会犯什么错）。所以，我们先生成DAG，检查DAG，DAG检查通过以后，再根据DAG生成incomplete proof。解释，DAG里面的节点，边，都是什么意思，还有哪些附加信息（判断一下是否是本质的东西，是否需要说）。为什么是DAG不是tree（提及我们的图）。解释，对DAG的检查都做了什么。


\item  每个subagent都拿着整个incomplete proof去操作，但是就证它自己要证的那一块。讲一下这个问题是怎么解决的。对每个subagent要证的admit加上ID来帮助识别他们。

\end{itemize}
\end{comment}

\ljy{If a decomposition remains only in the primary agent's free-form
reasoning, it cannot serve as a reliable basis for the subsequent
proof process. The proof logic underlying the decomposition is
implicit in the LLM's reasoning, where a necessary premise may be
overlooked, an unsupported dependency may be assumed, or a subgoal may
be introduced even though its result does not contribute to the
original lemma. Because this logic has no explicit representation, the
system cannot mechanically inspect the exact subgoals, their
dependencies, or how their results are intended to contribute to the
original lemma before proof construction begins.

In our preliminary attempts, we asked the primary agent to directly
translate such an implicit decomposition into an incomplete Rocq proof
in which the proofs of the proposed subgoals were temporarily replaced
by \texttt{admit}. This approach performed poorly because the LLM had
to determine the decomposition and encode it as an ordered Rocq proof
at the same time. For example, in
Figure~\ref{fig:decomp_example}, proving
\texttt{S1} does not establish
\texttt{H1} unless the decomposition also provides
\texttt{S2}. If \texttt{S2} is omitted and
\texttt{H1} is treated as a composition node, the generated proof
sketch cannot derive \texttt{H1}. If the gap is instead hidden by
placing an \texttt{admit} at \texttt{H1}, the subagent receives a
larger proof obligation that the intended decomposition has failed to
simplify. Such errors lead to repeated revisions of the proof sketch
or ineffective subagent attempts.

To make the proposed decomposition explicit and mechanically
checkable before it is encoded as Rocq code, ProsaBuddy requires the
primary agent to first represent it as a directed acyclic graph (DAG),
called a proof plan. Each node records a subgoal as a Rocq proposition,
and a directed edge from node \(u\) to node \(v\) means that the result
of \(u\) may be used when proving \(v\). The plan also records the
target lemma and assigns each node a unique identifier, making the
subgoals and their dependencies unambiguous.
The plan further specifies how each node is materialized in the proof
sketch. For a composition node, the primary agent writes complete Rocq
commands that derive the node's conclusion from its predecessor
results. By contrast, a delegation candidate represents a
proof obligation whose proof is left open in a proof region and
assigned to a subagent. A delegated node may still depend on and use
predecessor results. Thus, the distinction specifies whether a node is
established during proof-sketch construction or remains to be proved
by a subagent; it is not determined solely by the node's position in
the DAG. The unique identifier of each
delegation candidate is subsequently used to associate it
with its corresponding proof region. Figure~\ref{fig:decomp_example} illustrates this distinction.
The proofs of \texttt{S1}, \texttt{S2}, and \texttt{H2} are left as
\texttt{admit}, so these nodes are marked as
delegation candidate. In contrast, \texttt{H1} is a
composition node because its conclusion is derived by the complete
command \texttt{leq\_trans S1 S2}. The target lemma is similarly
completed by combining \texttt{H1} and \texttt{H2} with
\texttt{leq\_add}. Although the proofs of the predecessor nodes remain
unfinished, Rocq can already check that their stated results are
sufficient to construct \texttt{H1} and the final target.In particular,
\texttt{H2} demonstrates that a delegation candidate may have a
predecessor: it may use the validated result \texttt{H1}, but its
remaining proof is still left to a subagent.
A DAG is used instead of a tree because an intermediate result may be
used by more than one later proof step. With dependencies directed from
a result to the nodes that use it, a tree would allow each non-root
result to have only one parent, forcing the plan either to duplicate a
shared subgoal or to omit one of its uses. A DAG represents such
sharing directly while excluding circular dependencies.


Before generating the incomplete proof, ProsaBuddy checks that the
submitted plan refers to the intended target lemma by comparing its
recorded name and conclusion with the Rocq source. It then checks that
node identifiers are unique, that every dependency edge refers to
declared nodes, and that the dependency graph contains no cycle. These
checks reject malformed or internally inconsistent dependencies before
they are encoded as Rocq proof commands.

In addition to its subgoal and dependencies, a plan node may record a
library lemma that the primary agent proposes to use. This is
node-level proof information rather than part of the DAG's dependency
structure. A structurally valid proof plan may nevertheless rely on an
invalid use of such a lemma. The LLM may refer to a lemma that is
unavailable in the current environment or overlook premises required
for applying it. In either case, the corresponding node remains
unsupported even though the dependency graph is well formed.
ProsaBuddy therefore uses Rocq to validate the candidate lemma in the
current proof context and, when the plan relies on it to establish a
node, checks that its required premises are provided by the context or
by the node's declared dependencies. A plan containing an unavailable
or unsupported candidate lemma is rejected before proof construction.
This check does not prove the node; it only ensures that the planned
use of the library lemma is consistent with the recorded proof plan.

After the proof plan passes these checks, the primary agent materializes
it as an incomplete Rocq proof. A composition node is represented by
complete Rocq commands, whereas each
delegation candidate is represented by a proof region whose
proof block initially contains \texttt{admit}. ProsaBuddy then compiles
the complete proof sketch. This compilation checks that the planned
subgoals are well-typed in their local contexts and that, assuming the
delegated subgoals are eventually proved, the composition nodes derive
the intermediate results and close the original goal.

These checks provide only a conditional guarantee. The proof-plan
check validates the recorded dependency structure, while compilation
of the incomplete proof checks that the original lemma follows if all
delegated subgoals are proved. It does not establish that these
subgoals are themselves provable. Full correctness is obtained only
after every \texttt{admit} has been replaced by a Rocq-checked proof
and the complete target proof passes final validation.
}

\ljy{Each subagent receives the complete incomplete proof but is responsible
for proving only one assigned subgoal. Providing the complete proof is
necessary because a delegated subgoal may depend on local variables,
hypotheses, and intermediate results available only at its position in
the original proof. Extracting it as a separate global lemma would
require reconstructing this local context and could change the proof
obligation seen by the subagent. Keeping the subgoal in place instead
allows the subagent to work with the same context in which its result
will eventually be used.

This design introduces an identification and isolation problem. The
incomplete proof may contain several similar \texttt{admit}
placeholders, and their positions may change as the primary agent
refines the decomposition or advances the proof. Referring to the
$i$-th \texttt{admit} therefore does not reliably identify the
assigned subgoal. ProsaBuddy addresses this problem by associating each
delegated \texttt{admit} with a unique identifier and giving the
subagent the identifier of the subgoal it must prove. The subagent may
inspect the complete proof for context but may modify only the proof
block associated with that identifier. After the subagent returns,
ProsaBuddy accepts the result only if the assigned block has been
updated without modifying the other parts of the proof. This allows
subagents to use the complete local context while preventing them from
solving the wrong \texttt{admit} or interfering with other proof
tasks.}






!!!!!!!!!!!!!!!!!!!


\tochange{A proof region consists of
annotations written as Rocq comments and the Rocq source
delimited by these comments. The annotations identify the
region, the subgoal assigned to the subagent, and the previously
established results that the subgoal may use. ProsaBuddy reads
these annotations, whereas Rocq ignores them. The proof block initially contains an
\texttt{admit} placeholder and is subsequently completed by
the assigned subagent. The annotations are omitted from
Figure~\ref{fig:decomp_example} for brevity. This representation
does not change how the primary agent decomposes the target
lemma; it only identifies the part of the Rocq proof sketch
assigned to each subagent.}


==> sections/discussion.tex <==
\section{Discussions}

1.  soundness check

Rango: Adaptive Retrieval-Augmented Proving for Automated Software Verification

The proof attempt will be
in one of three states: complete, invalid, or incomplete. If
the proof attempt is complete, meaning that Coq shows no
more goals to be proven, then the search is successful. If
the proof attempt is invalid, then the tactic sampled from the
language model resulted in an error, and the searcher begins a
new rollout. If the proof attempt is incomplete, the searcher
continues the current rollout by sampling yet another tactic
from the tactic generator

https://rocq-prover.org/doc/V9.2.0/refman/proofs/writing-proofs/proof-mode.html

valid proof : Qed., Defined./ Defined ident., Save ident., Proof term. 

invalid proof: Admitted., Abort., Abort All.,


The Rocq compiler and the Checker mechanism serve
complementary purposes. When the current \texttt{.v} file
successfully compiles, Rocq elaborates the generated tactic
script into a proof term and checks this term using the Rocq
kernel. For a theorem closed with \texttt{Qed.}, successful
compilation establishes that the generated proof term has the
type declared by that theorem in the environment constructed
from the current file. Compilation does not, however, determine
whether the agent has changed the theorem declaration or the
source from which that environment was constructed.

In ProsaBuddy, Checker denotes a collection of script-based
checks that are applied throughout proof construction, rather
than a single tool that is invoked only after the proof has
been generated. At the beginning of a proof task, these checks
identify the target file and target theorem. They also record
the target theorem declaration and the source text outside its
proof. This information determines which part of the file the
agent is permitted to edit.

Every subsequent edit to the target file is checked before it
is accepted. The source before the target proof and the source
after its proof terminator must remain unchanged. Consequently,
the agent cannot change the theorem name, parameters,
hypotheses, or conclusion. It also cannot modify imports,
preceding definitions, other theorem declarations, or the
source following the target proof. The target file cannot be
replaced by another file or moved to another path. An edit
based on an earlier version of the source is rejected until the
agent reads the current version and constructs a new edit.

The checks also require the target proof to retain a
well-formed boundary. It must contain exactly one
\texttt{Proof.} command followed by exactly one proof
terminator, and no tactic or command may occur after that
terminator within the target proof. When a subagent is assigned
a \texttt{proof\_region}, a narrower check permits it to modify
only the Rocq source enclosed by that region. Text outside the
assigned region, including the proof commands that combine
its result with other subgoals, must remain unchanged.

The agent may introduce tactics and local facts inside the
authorized proof text. For example, it may use
\texttt{have}, \texttt{assert}, or a local \texttt{let}
binding to establish an intermediate result. These local facts
remain part of the target proof and are checked by Rocq when
the proof script is elaborated. They do not modify the target
theorem statement or introduce a new global assumption. In
addition, the file-system sandbox prevents the agent from
modifying imported libraries, project configuration, or other
modeling files.

The same checks are applied again when ProsaBuddy determines
whether the proof task has succeeded. Under the success
criterion used by ProsaBuddy, the target proof must end with
\texttt{Qed.}, must contain no \texttt{admit}, empty proof
block, \texttt{Admitted.}, or \texttt{Abort.}, and the complete
generated file must pass Rocq compilation. Although Rocq also
accepts proofs terminated by \texttt{Defined.}, the current
ProsaBuddy success check requires \texttt{Qed.}.

A subagent success report or a validation certificate for an
individual \texttt{proof\_region} is only an intermediate
result. The proof task is counted as successful only after the
complete target proof satisfies the editing-scope checks, the
unfinished-proof checks, and Rocq compilation. Thus, the
script-based Checker checks preserve the original theorem and
its environment, while the Rocq kernel verifies the proof
written for that theorem.

2. releated works


NLIR: Natural Language Intermediate Representation for Mechanized Theorem Proving (NIPS workshop 2024 open source)

Agentic Verification of Software Systemst(AutoRocq)(arxiv 2026 Mar, FSE2026,  open source 2026 Mar, the baseline of it is palm,copra,rango)

Automated Lemma Discovery in Agentic Program Verification(arxiv 2026 Mar v1, 2026 Jul v2, ASE2026, open source Jul 2026, the baseline is AutoRocq)

Cobblestone: A Divide-and-Conquer Approach for Automating Formal Verification (arxiv 2024 ICSE2026, open source, the baseline is PALM,RANGO)

Proof Repair Utilizing Large Language Models: A Case Study on the Copland Remote Attestation Proofbase(AISoLA 2024, open source, interactive with human)


Harnessing Code Agents for Automatic Software Verification(arxiv 2026 Jul, open source, the baseline is AutoRocq, claudecode+harness)








LLM-Enhanced Theorem Proving with Term Explanation and Tactic Parameter Repair(Internetware 2024 copra+two models, not open source)

Adaptive Proof Refinement with LLM-Guided Strategy Selection(arxiv 2025, ASE 2026, not open source)

Clarifying Before Reasoning: A Coq Prover with Structural Context(arxiv 2025, not open source)


Planning to Hammer: Difficulty-Aware Decomposition for Automating Rocq Proofs(arxiv 2020 Jul, OOPSLA 2026, not open 


\ljy{section III-A overview

The primary agent first records the decomposition as a structured
proof plan. The plan is represented as a directed acyclic graph
(DAG): each node records a subgoal stated in Rocq syntax, and an edge
from node $A$ to node $B$ states that the result established for $A$
is required to prove $B$. A node that the primary agent proposes to
assign to a subagent is marked as a
\texttt{delegation\_candidate}.
After the system mechanically checks the plan, the primary agent writes each
node marked as a \texttt{delegation\_candidate} into the Rocq proof
sketch as a \texttt{proof\_region}. After the plan passes the mechanical checks described in
Section~III-B, the primary agent represents every
\texttt{delegation\_candidate} node by exactly one
\texttt{proof\_region} in the Rocq proof sketch. A
\texttt{proof\_region} consists of annotations encoded as Rocq
comments and the Rocq source text delimited by these comments. The
annotations record the identity of the region and its correspondence
with the proof plan, including the target subgoal and its predecessor
nodes. These annotations are interpreted by ProsaBuddy but ignored
by Rocq. The delimited Rocq source states the assigned subgoal as a
named local assertion and contains the proof block for that assertion,
together with any helper facts introduced within the same region.
Before assigning a \texttt{proof\_region} to a subagent, the system
checks that its \texttt{plan\_node}, subgoal statement, and
\texttt{depends\_on} annotations agree with the corresponding node
in the proof plan, and that every node listed in
\texttt{depends\_on} has already been validated by Rocq for the
current version of the proof file. Section~III-B specifies the
remaining checks on the region annotations and the shape of its
subgoal.}

\ljy{section III-B
Before the primary agent writes a Rocq proof sketch following the
proof plan, ProsaBuddy mechanically checks the structure of the plan.
It verifies that the theorem name and conclusion recorded in the plan
match the target lemma in the source file. It also checks that each
node has a unique identifier, that both endpoints of every dependency
edge are nodes declared in the plan, and that the dependency graph
contains no cycle. For a node that combines several predecessor
results or completes the original lemma, the plan records which
predecessor results are used and the conclusion established by their
combination.

After these checks pass, the primary agent writes the Rocq proof
sketch. Each node marked as a \texttt{delegation\_candidate} must be
represented by exactly one \texttt{proof\_region}. The proof block
for the assigned subgoal initially contains an \texttt{admit}
placeholder. The primary agent also writes the Rocq tactics outside
the regions that use these results by name, such as \texttt{H1} and
\texttt{H2} in Figure~\ref{fig:decomp_example}, to complete the proof
of the original lemma.

ProsaBuddy then invokes the Rocq compiler on the complete proof
sketch. The compiler checks that each subgoal statement is a
well-typed Rocq proposition under the variables and hypotheses
available at the point where it is introduced. It also type-checks
the tactics outside the regions and verifies that they close all
other goals, including the final goal of the original lemma. This
compilation does not prove a subgoal whose proof block still contains
\texttt{admit}; such subgoals are subsequently assigned to subagents.}

\ljy{section III-B
\subsubsection{Plan Review and Candidate-Lemma Auditing}

Before editing the target proof, the primary agent submits the proof
plan through the \texttt{proof\_plan} tool. The tool locates the
target lemma from the current position in the \texttt{.v} file and
reads its name and conclusion from the source file. ProsaBuddy then
compares them with the lemma name and conclusion recorded in the
submitted plan. The plan is rejected if either of them differs. Each
node records a subgoal, the predecessor nodes on which it depends,
and whether it is marked as a \texttt{delegation\_candidate}. The plan
also records any existing lemmas that the primary agent proposes to
use for proving the node.

ProsaBuddy then mechanically checks the structure of the plan. It
checks that every node has a unique identifier and that every
identifier listed in \texttt{depends\_on} refers to a node declared
in the plan. It also rejects a plan whose dependency graph contains
a cycle.
The tool reports \emph{ready} when it finds neither a blocking error
nor a warning. It reports \emph{revise} when the plan has no blocking
error but contains information that should be reconsidered. A
\emph{revise} result does not prevent the primary agent from writing
the Rocq proof sketch. The tool reports \emph{reject} when it finds a
blocking error; a rejected plan cannot be used to write the proof
sketch.
When the plan has no blocking error, ProsaBuddy stores it for the
target lemma. After the primary agent writes the proof sketch, the
system compares the \texttt{plan\_node}, target subgoal, and
\texttt{depends\_on} annotations of every \texttt{proof\_region} with
the stored plan. This check determines whether each region corresponds
to the reviewed plan node and records the same predecessor
dependencies.

A candidate lemma is an existing lemma from Prosa, MathComp, or the
current source file that the primary agent proposes to use when
proving a plan node. For a candidate that the primary agent intends
to apply directly, ProsaBuddy first invokes Rocq with
\texttt{Check} to determine whether the lemma is available and to
obtain its actual type.
ProsaBuddy then constructs a temporary Rocq proof containing the
imports, variables, and hypotheses available at the target theorem.
It states the subgoal of the plan node in this context and applies
the candidate lemma using \texttt{eapply}. It subsequently attempts
to solve straightforward subgoals using \texttt{assumption} and
\texttt{reflexivity}. Any Rocq subgoal that remains after these
tactics corresponds to a premise of the candidate lemma that is not
provided by the current theorem context.
If no subgoal remains, the candidate can be applied directly in the
current context. Otherwise, every remaining subgoal must correspond
to the subgoal of a predecessor node listed in
\texttt{depends\_on}, or must already have been proved in a
\texttt{proof\_region} validated by Rocq for the current version of
the source file. If neither condition holds, the candidate lemma
does not support the dependencies declared for the node.
For a candidate that is intended only for rewriting or for proving
an auxiliary fact, the planning-stage audit uses \texttt{Check} to
confirm that the lemma is available. The correctness of its concrete
use is checked later by Rocq when the proof sketch or the corresponding
\texttt{proof\_region} is compiled.
Passing this audit does not prove the plan node. It only confirms that
the candidate lemma is available and, for direct application,
identifies the additional subgoals that its application would create.
}

\ljy{SECTION III-B
\subsubsection{Proof-Region Lifecycle and Evidence-Guided Repair}
A \texttt{proof\_region} corresponding to a
\texttt{delegation\_candidate} is not assigned immediately.
Before launching a subagent, ProsaBuddy checks whether the
region contains enough information to define the assigned
task.The region markers must enclose the Rocq statement of the
assigned subgoal together with its complete proof block. The
\texttt{source} annotation records where the proposed proof
step originated. The \texttt{input} annotation lists the facts
expected to be available to the region, while
\texttt{output} identifies the named result established by the
region. The \texttt{expected} annotation describes the
intended result of the local proof step, and
\texttt{normal\_form} records the expected textual form of the
target proposition.

ProsaBuddy records one of six states for each
\texttt{proof\_region}. A \emph{pending} region still contains
an unfinished proof block and is waiting for its dependencies
or for assignment. A region becomes \emph{running} when it is
assigned to a subagent. A \emph{split} region has been divided
by that subagent into smaller proof blocks inside the same
region. The same subagent task continues to process these
blocks; the split does not create new theorem-level plan nodes
or launch additional lemma-proving subagents.
A region becomes \emph{unvalidated} when its
\texttt{admit} placeholder or empty proof block has been
removed, but the resulting source has not yet been validated
by the Rocq compiler. It becomes \emph{solved} only after the
compiler validates the current version of the region and
ProsaBuddy records a validation certificate. Finally, a region
is marked \emph{escalated} when the subagent reports that the
assigned subgoal cannot be completed without changing the
subgoal statement, adding a missing predecessor result, or
editing proof commands outside the assigned region. Such a
region is returned to the primary agent for revision.

A validation certificate records that the Rocq compiler has
validated a particular version of a \texttt{proof\_region}.
It contains the normalized file path, the
\texttt{admit\_id}, a digest of the region text, a hash of the
normalized source prefix ending at the region, an identifier
for the compiler result, the validator that produced the
record, and the validation time. The certificate remains
current only while the file, region identifier, region text,
and preceding source context still match these recorded
values. Editing the region or the source preceding it therefore
invalidates the certificate.

A pending region can be assigned only when every identifier
in its \texttt{depends\_on} field that refers to another
\texttt{proof\_region} is in the \emph{solved} state with a
current certificate. References to variables, hypotheses, or
other facts already available in the theorem context do not
create scheduler dependencies. ProsaBuddy assigns one ready
region at a time. When several pending regions have all their
dependencies satisfied, their order in the source file is used
to select the next region; source order does not introduce an
additional dependency.

After launching a subagent, the primary agent suspends and
waits for the subagent to return. The subagent returns either
a proof of the assigned subgoal or a failure report. A failure
report explains why the current attempt did not complete the
subgoal and identifies any assumption, intermediate result, or
change to the decomposition that the subagent considers
necessary.

ProsaBuddy retains these failure reports and makes the
relevant reports available to the primary agent when it later
refines the same proof. Consequently, the primary agent does
not have to treat each refinement as an independent attempt.
It can use the missing information identified in an earlier
report to introduce additional subgoals, change the boundary
of the failed subgoal, or select a different existing lemma.
The retained reports also help the primary agent avoid
repeating a decomposition that has already failed in the same
proof state.
A failure report is used as guidance for subsequent
decomposition; it is not a proof that the assigned subgoal is
unprovable. A previously unsuccessful approach may therefore
be reconsidered after the decomposition has changed or after
the missing intermediate result has been established. When
the primary agent revises the decomposition, subgoals that
have already been proved are retained.

}

\ljy{section III-D
In addition to the three Rocq interfaces, ProsaBuddy
provides two external tools for managing the decomposition
workflow: \texttt{proof\_plan} and \texttt{checkpoint}.
Before the primary agent writes the Rocq proof sketch, the
\texttt{proof\_plan} tool compares the theorem name and
conclusion recorded in the plan with the target lemma in the
source file. It also checks the structure of the dependency
graph and audits the candidate lemmas proposed for individual
plan nodes. After the proof sketch has been written,
ProsaBuddy compares the annotations of each
\texttt{proof\_region} with the stored plan and checks whether
the region contains the information required for assignment
to a subagent.

At a proof milestone, the primary agent calls
\texttt{checkpoint}, which invokes the Rocq compiler on the
current source. The compilation result is used to update the
state of each \texttt{proof\_region}, create or invalidate its
validation certificate, and classify whether the latest edit
constitutes proof progress. Passing the
\texttt{proof\_plan} checks or the checks performed before
delegation does not prove a subgoal. A region is marked
\emph{solved} only after its current version has been
validated by Rocq. Thus, the LLM proposes the lemma
decomposition and writes the proof text, while ProsaBuddy
checks the plan and region structure and records the results
of Rocq validation.
}

\ljy{section III-D
\textbf{Checkpoint and progress guard.}
We expose \texttt{checkpoint} as an external tool for
validating intermediate proof states. At a proof milestone,
the tool invokes the Rocq compiler on the current staged
source. In addition to reporting the compilation result and
the first compiler error, it updates the states of the
\texttt{proof\_region} blocks and determines whether the
current edit constitutes proof progress.

For this purpose, the tool counts unfinished constructs in the
target theorem, including \texttt{admit} placeholders, empty
proof blocks, and proofs terminated by \texttt{Admitted} or
\texttt{Abort}. It also checks whether the theorem ends with
\texttt{Qed} and counts the \texttt{proof\_region} blocks that
do not have a current validation certificate.

The tool classifies the result as \emph{hard},
\emph{structural}, or \emph{debug} progress. Hard progress is
recorded when compilation produces a new region certificate,
when the number of unresolved regions decreases and every
removed region has a current certificate, or when the complete
target theorem passes the final \texttt{Qed} check. Structural
progress records that an accepted decomposition has been
written as dependency-complete regions and that the resulting
proof sketch compiles, but it does not claim that any new
subgoal has been proved. Debug progress records diagnostic
movement, such as the first compiler error occurring later in
the proof. Removing a syntactic placeholder without obtaining
a compiler certificate is not classified as hard proof
progress.

The agent runtime uses these progress records to prevent
repeated work on an unchanged blocker. It monitors consecutive
tool calls without hard progress, repeated compiler-result
signatures, and repeated subagent attempts on the same theorem
and region. After repeated attempts without a new compiler-
backed progress record, the runtime first warns the agent and
can subsequently prevent another proof-producing subagent
from being launched for the unchanged blocker. Changes only
to comments, region identifiers, whitespace, or other
administrative text do not release this restriction. A new
compiler-backed progress record, or a substantive change to
the proof step under repair, allows the workflow to be
reconsidered.

This mechanism is distinct from the final Checker. The
checkpoint tool and progress guard control intermediate proof
construction and repeated agent actions, whereas the Checker
audits the final proof file against the original file.}

\ljy{experiment}
\begin{table}[htbp]
\caption{Results for multiple runs}
%\guan{change the format, make it consistent with other tables}
\centering
\tiny
\renewcommand{\arraystretch}{1.6}
\begin{tabular}{cccccccc}
% \hline
\toprule
 & 1 & 2 & 7 & 8 & 17 & 22  \\
\hline

% rocqstar level2 is old 10
PALM & 0/5 & 0/5 & 0/5 & 0/5 & 0/5 & 0/5
RocqStar & 0/5 & 0/5 & 0/5 & 0/5 & ? & 0/5  \\
OpenCode & 0/5 & 0/5 & 0/5 & 0/5 & 2/5 & 0/5 & - \\
\textbf{\ours} & 4/5 & 4/5 & 5/5 & 5/5 & 5/5 & 4/5  \\
    \midrule 
% only run those who are not completed by opencode
pass@1 of Prosabuddy & 0.8 & 
0.8 & 1 & 1 & 1 & 0.8  \\
pass@3 of Prosabuddy & 1 & 
1 & 1 & 1 & 1 & 1  \\
Token Range & 29,168-54,525 & 
35,546-64,957 & ? & 13,077-38,724 & ? & 22,890-31,614  \\
Average Token & 44,171 & 
50,630 & ? & 25,220 & ? & 28,120  \\
% %31 & - & - & - & - & - \\
% \hline
\bottomrule
\end{tabular}
~\\
\footnotesize
\label{tab:multiple}
\end{table}













\guan{Guan to do list:
\begin{itemize}
\item Qwen3.7-Max??
\end{itemize}
}

\guan{Challenges:
\begin{itemize}
\item Parameterized lemma
\item furthermore, this lead to too many goals: Prosa proofs tend to introduces too many lemma or deduction  

\item missing knowledge: new concept????

case discussion: subgoal

\end{itemize}
}

\subsection{ProsaBuddy is Interactive}
In the 

\subsection{Autoformalization}

==> sections/preparation.tex <==
\section{Prepare Your Paper Before Styling}
Before you begin to format your paper, first write and save the content as a 
separate text file. Complete all content and organizational editing before 
formatting. Please note sections \ref{AA} to \ref{FAT} below for more information on 
proofreading, spelling and grammar.

Keep your text and graphic files separate until after the text has been 
formatted and styled. Do not number text heads---{\LaTeX} will do that 
for you.

\subsection{Abbreviations and Acronyms}\label{AA}
Define abbreviations and acronyms the first time they are used in the text, 
even after they have been defined in the abstract. Abbreviations such as 
IEEE, SI, MKS, CGS, ac, dc, and rms do not have to be defined. Do not use 
abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}
\begin{itemize}
\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as ``3.5-inch disk drive''.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: ``Wb/m\textsuperscript{2}'' or ``webers per square meter'', not ``webers/m\textsuperscript{2}''. Spell out units when they appear in text: ``. . . a few henries'', not ``. . . a few H''.
\item Use a zero before decimal points: ``0.25'', not ``.25''. Use ``cm\textsuperscript{3}'', not ``cc''.)
\end{itemize}

\subsection{Equations}
Number equations consecutively. To make your 
equations more compact, you may use the solidus (~/~), the exp function, or 
appropriate exponents. Italicize Roman symbols for quantities and variables, 
but not Greek symbols. Use a long dash rather than a hyphen for a minus 
sign. Punctuate equations with commas or periods when they are part of a 
sentence, as in:
\begin{equation}
a+b=\gamma\label{eq}
\end{equation}

Be sure that the 
symbols in your equation have been defined before or immediately following 
the equation. Use ``\eqref{eq}'', not ``Eq.~\eqref{eq}'' or ``equation \eqref{eq}'', except at 
the beginning of a sentence: ``Equation \eqref{eq} is . . .''

\subsection{\LaTeX-Specific Advice}

Please use ``soft'' (e.g., \verb|\eqref{Eq}|) cross references instead
of ``hard'' references (e.g., \verb|(1)|). That will make it possible
to combine sections, add equations, or change the order of figures or
citations without having to go through the file line by line.

Please don't use the \verb|{eqnarray}| equation environment. Use
\verb|{align}| or \verb|{IEEEeqnarray}| instead. The \verb|{eqnarray}|
environment leaves unsightly spaces around relation symbols.

Please note that the \verb|{subequations}| environment in {\LaTeX}
will increment the main equation counter even when there are no
equation numbers displayed. If you forget that, you might write an
article in which the equation numbers skip from (17) to (20), causing
the copy editors to wonder if you've discovered a new method of
counting.

{\BibTeX} does not work by magic. It doesn't get the bibliographic
data from thin air but from .bib files. If you use {\BibTeX} to produce a
bibliography you must send the .bib files. 

{\LaTeX} can't read your mind. If you assign the same label to a
subsubsection and a table, you might find that Table I has been cross
referenced as Table IV-B3. 

{\LaTeX} does not have precognitive abilities. If you put a
\verb|\label| command before the command that updates the counter it's
supposed to be using, the label will pick up the last counter to be
cross referenced instead. In particular, a \verb|\label| command
should not go before the caption of a figure or a table.

Do not use \verb|\nonumber| inside the \verb|{array}| environment. It
will not stop equation numbers inside \verb|{array}| (there won't be
any anyway) and it might stop a wanted equation number in the
surrounding equation.

\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
\item The word ``data'' is plural, not singular.
\item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
\item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
\item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
\item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
\item Do not confuse ``imply'' and ``infer''.
\item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
\item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}
An excellent style manual for science writers is \cite{b7}.

\subsection{Authors and Affiliations}\label{AAA}
\textbf{The class file is designed for, but not limited to, six authors.} A 
minimum of one author is required for all conference articles. Author names 
should be listed starting from left to right and then moving down to the 
next line. This is the author sequence that will be used in future citations 
and by indexing services. Names should not be listed in columns nor group by 
affiliation. Please keep your affiliations as succinct as possible (for 
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}\label{ITH}
Headings, or heads, are organizational devices that guide the reader through 
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not 
topically subordinate to each other. Examples include Acknowledgments and 
References and, for these, the correct style to use is ``Heading 5''. Use 
``figure caption'' for your Figure captions, and ``table head'' for your 
table title. Run-in heads, such as ``Abstract'', will require you to apply a 
style (in this case, italic) in addition to the style provided by the drop 
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For 
example, the paper title is the primary text head because all subsequent 
material relates and elaborates on this one topic. If there are two or more 
sub-topics, the next level head (uppercase Roman numerals) should be used 
and, conversely, if there are not at least two sub-topics, then no subheads 
should be introduced.

\subsection{Figures and Tables}\label{FAT}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and 
bottom of columns. Avoid placing them in the middle of columns. Large 
figures and tables may span across both columns. Figure captions should be 
below the figures; table heads should appear above the tables. Insert 
figures and tables after they are cited in the text. Use the abbreviation 
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words 
rather than symbols or abbreviations when writing Figure axis labels to 
avoid confusing the reader. As an example, write the quantity 
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including 
units in the label, present them within parentheses. Do not label axes only 
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization 
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of 
quantities and units. For example, write ``Temperature (K)'', not 
``Temperature/K''.


==> sections/relatedworks.tex <==
\section{Related Works}\label{relatedworks}

\subsection{PROSA}

PROSA was introduced as a Coq-based foundation for verified real-time scheduling theory~\cite{prosa}. It emphasizes readable specifications, explicit assumptions, and proof reuse. The initial development used discrete time, opaque job and task types, and fine-grained hypotheses. It mechanized representative results such as multiprocessor response-time analysis, global fixed-priority RTA with release jitter, parallel-task analysis, and an EDF dominance theorem. This showed that nontrivial scheduling theory could be checked mechanically.

Later work extended PROSA and related verified scheduling infrastructure in several directions. These include sustainability theory and weak sustainability~\cite{strongweaksustainability}, Abstract Response-Time Analysis based on the busy-window principle~\cite{aRTA}, FIFO response-time analysis with arbitrary deadlines and arrival curves~\cite{intuition2coq}, POET certificates for response-time bounds from YAML task-set descriptions~\cite{pOET}, connections between response-time analysis and Network Calculus~\cite{linkRandNc}, and links between PROSA and verified C scheduler implementations through RefinedC~\cite{refinedProsa}.

Together, these works make PROSA a useful infrastructure for verified real-time systems. They provide a common formal language for scheduling models, assumptions, and response-time theorems, and they support proof reuse across scheduling policies and analysis styles. At the same time, PROSA still covers only part of real-time scheduling theory. New theorems often require expert proof engineering, carefully stated assumptions, reusable abstractions, and library-specific proof patterns. Thus, PROSA improves reliability, but it also exposes a bottleneck: mechanized schedulability proofs remain difficult to construct and maintain.

% \subsection{Pre-LLM Theorem Proving Automation}

% Before the rise of LLM-based theorem proving, Coq/Rocq had already accumulated a rich ecosystem of automation techniques for reducing manual proof effort. At the most immediate level, Coq provides tactic-level automation for routine proof obligations. General-purpose tactics such as \texttt{auto}, \texttt{eauto}, \texttt{intuition}, \texttt{firstorder}, and \texttt{congruence} search through hypotheses and hint databases, while domain-specific procedures such as \texttt{omega}, \texttt{lia}, \texttt{nia}, \texttt{micromega}, \texttt{ring}, and \texttt{field} automate arithmetic and algebraic reasoning. These tactics are indispensable in large developments, but their scope is mostly local: they solve isolated subgoals once the surrounding proof structure has already been supplied by the user.

% Building on Coq's computational foundation, another major line of work developed proof by reflection. SSReflect \cite{ssreflect} and Mathematical  Components \cite{mathcomp} use boolean reflection, structured rewriting, canonical structures, and algebraic hierarchies to make recurring proof patterns reusable and efficient. CoqEAL \cite{coqeal} further explored how efficient computational algorithms can be connected to proof-oriented specifications. This reflective style is powerful because computation remains within Coq's trusted logic, but it requires substantial proof-engineering effort, including reification procedures, verified decision procedures, and reflection-friendly library design.

% Coq automation was also extended by connecting the proof assistant to external automated reasoning tools. SMTCoq \cite{smtcoq} and smt4coq \cite{smt4coq} translate Coq goals to SMT solvers such as Z3 or CVC-style engines and reconstruct or check solver certificates inside Coq. CoqHammer \cite{coqhammer} brings hammer-style automation to Coq by combining premise selection, translation to first-order logic, ATP calls, and proof reconstruction. These tools substantially expand the reach of automation for first-order, equality, arithmetic, and SMT-supported reasoning. However, they remain sensitive to translation quality, premise selection, and reconstruction failures, especially when proofs involve dependent types, higher-order structure, complex induction, or domain-specific invariants.

% Alongside solver integration, Coq users and tool builders developed increasingly expressive ways to program automation directly inside the proof assistant. Ltac \cite{ltac} and its successors or alternatives, including Ltac2, Mtac/Mtac2 \cite{mtac,mtac2}, Coq-Elpi \cite{coqelpi}, and MetaCoq \cite{metacoq}, provide mechanisms for building domain-specific tactics, inspecting proof states, and manipulating Coq terms and proof terms. These systems made it possible to encode reusable proof strategies for mature verification projects, but they also shifted part of the burden from individual proof scripts to the engineering of proof infrastructure.

% Prior to LLMs, researchers further explored machine-learning guidance for Coq proof automation. ML4PG \cite{ml4pg} used learning techniques to identify similar proof patterns in Coq/SSReflect developments, while CoqGym \cite{coqgym} provided a large-scale dataset and environment for learning tactic prediction from real Coq proofs.
% Systems such as Tactician \cite{tactician}, Proverbot9001 \cite{proverbot9001}, and TacTok \cite{tactok}, as well as CoqGym neural baselines such as ASTactic \cite{coqgym}, investigated learned tactic prediction, local proof search, and semantics-aware proof synthesis. These approaches improved tactic ranking and proof-step suggestion, but they largely remained tied to local proof states and existing tactic interfaces.

% Taken together, pre-LLM Coq automation significantly reduced the burden of routine reasoning through tactics, reflection, SMT/ATP integration, metaprogramming, and learning-guided search. Yet these techniques did not fully close the gap between local proof automation and high-level proof engineering. Tasks such as decomposing large verification goals, inventing reusable lemmas, selecting abstractions, coordinating induction arguments, and maintaining proofs across evolving formal developments still largely depended on expert human guidance.
\subsection{Pre-LLM Theorem Proving Automation}

The bottleneck exposed by PROSA is not unique to real-time scheduling or to Coq/Rocq. Mechanized proofs are hard to construct and maintain across proof assistants, and pre-LLM automation has long been developed in systems such as Isabelle/HOL~\cite{sledgehammer}, HOL Light~\cite{hollight}, Lean~\cite{mathlib}, and Coq/Rocq~\cite{coq}.

In Coq/Rocq, pre-LLM automation covered tactics, reflection, solver integration, and programmable proof infrastructure. Basic tactics such as \texttt{auto}, \texttt{eauto}, \texttt{intuition}, \texttt{firstorder}, \texttt{congruence}, \texttt{omega}, \texttt{lia}, \texttt{nia}, \texttt{micromega}, \texttt{ring}, and \texttt{field} automate routine logical, arithmetic, and algebraic reasoning. SSReflect~\cite{ssreflect}, Mathematical Components~\cite{mathcomp}, and CoqEAL~\cite{coqeal} make recurring proof patterns reusable through reflection and proof-oriented computation. SMTCoq~\cite{smtcoq}, smt4coq~\cite{smt4coq}, and CoqHammer~\cite{coqhammer} connect Coq goals to external reasoning or proof reconstruction. Ltac/Ltac2~\cite{ltac}, Mtac/Mtac2~\cite{mtac,mtac2}, Coq-Elpi~\cite{coqelpi}, and MetaCoq~\cite{metacoq} support domain-specific tactics and reusable proof infrastructure.

Learning-guided automation added data-driven support for proof search~\cite{learning_guided_ar_survey}. In Coq/Rocq, ML4PG~\cite{ml4pg}, CoqGym~\cite{coqgym}, Tactician~\cite{tactician}, Proverbot9001~\cite{proverbot9001}, TacTok~\cite{tactok}, and ASTactic~\cite{coqgym} explored proof-pattern mining, tactic prediction, local proof search, and proof-step prediction.

These automation techniques substantially reduce routine proof effort, but they do not fully address high-level proof engineering. Large mechanized developments still require experts to decompose complex goals, formulate auxiliary lemmas, choose suitable abstractions, coordinate induction arguments, and maintain proofs as libraries evolve. 

% \subsection{Autoformalization}

% Pre-LLM Coq automation largely operates after a goal has been formalized: tactics, solvers, and proof-search tools try to discharge obligations that already exist inside the proof assistant. Autoformalization addresses a complementary problem: translating informal mathematical or specification-level content into machine-checkable formal artifacts. Its inputs may include theorem statements, requirements, proof outlines, or natural-language proofs, and its outputs may range from definitions and theorem statements to proof sketches or full proof scripts. This task has been studied through controlled languages, corpus-based translation, symbolic disambiguation, semantic parsing, neural translation, and, more recently, LLM-based methods.


% Early autoformalization work focused on connecting informal mathematical text with formal libraries and proof assistants without relying on large language models. Kaliszyk et al. \cite{informal_formal_translation} proposed corpus-based translation methods between informal and formal mathematics, framing autoformalization as a data-driven alignment problem between mathematical prose and formal corpora. Wang et al. \cite{neural_informal_formal} later explored neural translation from informal to formal mathematics, showing that sequence models could learn nontrivial mappings from mathematical text to formal expressions. M{\"u}ller and Kaliszyk \cite{symbolic_disambiguation} further studied the disambiguation of symbolic expressions in informal documents, addressing a key obstacle for formalization: informal mathematical notation is often underspecified and must be resolved before it can be translated into a formal language. These works establish autoformalization as a broader research problem that predates the current LLM-based setting. 

% Recent LLM-based work has expanded autoformalization across multiple target systems and application settings. For Coq/Rocq, directly relevant LLM-based work remains limited, but multi-language formalization efforts have begun to include Coq as a target system. Cao et al. \cite{informal_to_formal_requirements} construct instruction-style data for translating natural-language requirements into verifiable formal artifacts across Coq, Lean4, Dafny, ACSL, and TLA+, providing a formal-verification-oriented benchmark for LLM-based informal-to-formal translation. Beyond Coq/Rocq, Wu et al. \cite{autoformalization_llm} showed that LLMs can translate natural-language mathematical problems into formal specifications and use the resulting data to improve downstream theorem proving. ProofNet \cite{proofnet} pairs informal mathematical statements and proofs with formal theorem statements to evaluate faithful autoformalization. Draft, Sketch, and Prove \cite{draftsketch} translates informal proofs into formal proof sketches that guide proof search. RAutoformalizer \cite{rautoformalizer} emphasizes retrieving the right formal dependencies to avoid plausible but ill-formed formalizations. 
% Survey \cite{autoformalization_survey} summarizes datasets, target systems, evaluation methods, and application domains across this line of work.

% Autoformalization is adjacent to proof generation, but it differs in emphasis. Autoformalization centers on translating informal content into formal artifacts, so informal statements, specifications, or proofs are part of the task itself. Proof generation may use informal explanations or paper proofs when available, but it can also start from an already formalized theorem statement and construct a checker-accepted proof script from the formal goal, library context, and prover feedback. Thus, informal text is not a mandatory input for proof generation, which is the focus of the Coq/Rocq systems reviewed below.

% \subsection{LLM-based Autonomous Theorem Proving}
% \begin{itemize}
%     \item general ATP (including lean and others, how LLM-based ATP achieves impressive results)

%     \item specific to Coq/Rocq
% \end{itemize}

% Given a formal theorem statement, recent work has begun to use LLMs as proof-producing components for interactive theorem provers. This direction has been explored across several formal systems, from early generative neural provers for Metamath and Lean-style benchmarks~\cite{gptf,htps}, to retrieval-augmented and model-training approaches for Lean~\cite{leandojo,llemma,deepseekprover,leanstar,deepseekproverv2,kiminaprover}, and to Isabelle/HOL systems that combine language models with hammer-style automation or proof repair~\cite{thor,baldur}. Due to space constraints, we focus below on Coq/Rocq systems, which are most closely related to our evaluation setting.

% This setting is distinct from autoformalization: rather than translating informal mathematical content into formal statements or proof sketches, these systems assume that the theorem has already been formalized and address the subsequent task of constructing a machine-checkable proof. Compared with earlier tactic-based or solver-based automation, LLM-based systems can synthesize longer proof fragments, make use of intermediate proof-state information, and revise failed attempts based on compiler feedback. CoqPilot \cite{coqpilot} packages this capability as a Coq-oriented development assistant, generating candidate proofs inside the proof-engineering workflow. COPRA \cite{copra} formulates proof search as an in-context interactive process, where the model proposes tactics, observes proof-state feedback, and continues the proof through a dialogue with the prover. PALM \cite{palm} further shows that proof generation can be strengthened by a generate-then-repair architecture, where low-level proof errors produced by the model are analyzed and repaired using symbolic procedures. Together, these systems demonstrate that LLMs can act as practical proof-generation components for Coq-style environments, while remaining complementary to autoformalization methods that operate before the theorem-proving stage.

% More recent systems further combine proof generation with retrieval and multi-step
% interaction. Rango \cite{rango} retrieves relevant premises and similar proofs from the
% current Coq project at each proof step, showing that project-local retrieval can
% substantially improve proof synthesis. RocqStar \cite{rocqstar} and ReCent-Prover \cite{recentprover}
% extend this trend toward agentic proof automation, introducing planning,
% reflection, and strategy-aware retrieval into Rocq proof generation.


% \begin{table}[t]
% \centering
% \tiny
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand{\arraystretch}{0.95}
% \caption{Representative LLM-based theorem proving systems for Coq/Rocq. ``Avail.'' means the paper/tool is publicly available; ``Open'' means the implementation is open-source.}
% \label{tab:llm_proof_automation}
% \begin{tabular}{@{}lclccp{4.5cm}@{}}
% \hline
% Work & Year & Prover & Avail. & Open & Retrieval? \\
% \hline
% CoqPilot~\cite{coqpilot}
% & 2024 & Coq & Yes & Yes
% & Context theorem selection from completed proofs; Jaccard/distance ranker, non-RAG \\

% PALM~\cite{palm}
% & 2024 & Coq & Yes & No
% &  BM25 premise retrieval over project environment; retrieved premises/defs are appended to the prompt \\

% Rango~\cite{rango}
% & 2025 & Coq & Yes & No
% & Adaptive RAG at each proof step; retrieves relevant premises and similar proofs from the current project \\

% COPRA~\cite{copra}
% & 2023 & Coq & Yes & No
% & External lemma retrieval; retrieved lemmas are included with search history in the prompt \\

% RocqStar~\cite{rocqstar}
% & 2025 & Rocq & Yes & Yes
% & Similarity-driven premise retrieval; self-attentive embedder for premise selection \\

% ReCent-Prover~\cite{recentprover}
% & 2026 & Rocq & Yes & No
% & Planning-conditioned retrieval; retrieves lemmas/proofs according to LLM-generated proof plans rather than subgoal similarity \\
% \hline
% \end{tabular}
% \end{table}
\begin{table}[t]
\centering
\tiny
\setlength{\tabcolsep}{2.5pt}
\renewcommand{\arraystretch}{0.95}
\caption{Representative LLM-based Coq/Rocq theorem proving systems. ``Avail.'' denotes practical usability; ``Source'' denotes public source availability.}
\label{tab:llm_proof_automation}
\begin{tabular}{@{}lclccp{4.5cm}@{}}
\toprule
Work & Year & Prover & Avail. & Source & Retrieval? \\
\midrule
CoqPilot~\cite{coqpilot}
& 2024 & Coq & Yes & Yes
& Context theorem selection from completed proofs; Jaccard/distance ranker, non-RAG \\

PALM~\cite{palm}
& 2024 & Coq & Yes & Yes
& BM25 premise retrieval over project environment; retrieved premises/defs are appended to the prompt \\

COPRA~\cite{copra}
& 2024 & Coq & Yes & Yes
& External lemma retrieval; retrieved lemmas are included with search history in the prompt \\

RocqStar~\cite{rocqstar}
& 2025 & Rocq & Yes & Yes
& Similarity-driven premise retrieval; self-attentive embedder for premise selection \\

Rango~\cite{rango}
& 2025 & Coq & No & No
& Adaptive RAG at each proof step; retrieves relevant premises and similar proofs from the current project \\

ReCent-Prover~\cite{recentprover}
& 2026 & Rocq & No & No
& Planning-conditioned retrieval; retrieves lemmas/proofs according to LLM-generated proof plans rather than subgoal similarity \\
\bottomrule
\end{tabular}
\end{table}
\subsection{LLM-based Autonomous Theorem Proving}

LLMs have recently been used for autoformalization and autonomous proof generation across several proof assistants. Recent surveys summarize this line of work~\cite{autoformalization_survey,llm_atp_survey}. Existing work covers Coq/Rocq~\cite{coqpilot,copra,palm,rango,rocqstar,recentprover}, Lean~\cite{autoformalization_llm,draftsketch,rautoformalizer,leandojo,llemma,legoprover,deepseekprover,lin2025leanstar,leancopilot,goedelprover,hilbert}, and Isabelle/HOL~\cite{thor,baldur,poetry}. 

For Coq/Rocq, recent LLM-based work mainly assumes formalized theorem statements and targets proof-script synthesis. CoqPilot~\cite{coqpilot} provides a Coq-oriented assistant implemented as a VS Code extension, where users mark proof holes with \texttt{admit}, configure completion services, and invoke the tool inside an open Coq file to generate, check, and substitute candidate proofs through \texttt{coq-lsp} during interactive editing. COPRA~\cite{copra} formulates proof search as an in-context interactive process where the model proposes tactics and observes proof-state feedback. PALM~\cite{palm} uses a generate-then-repair architecture to analyze and repair low-level proof errors. More recent systems combine proof generation with retrieval and multi-step interaction. Rango~\cite{rango} retrieves relevant premises and similar proofs from the current Coq project. RocqStar~\cite{rocqstar} and ReCent-Prover~\cite{recentprover} further introduce planning, reflection, and strategy-aware retrieval into Rocq proof generation. 
Table~\ref{tab:llm_proof_automation} summarizes representative Coq/Rocq-specific systems and their retrieval strategies.

Beyond these proof-assistant-specific systems, general-purpose LLM backbones and coding-agent harnesses can also support proof development. GPT, DeepSeek, Gemini, Claude, and coding agents such as OpenCode~\cite{opencode} can edit proof files, invoke Rocq, inspect errors, and repair proof scripts.

Overall, this body of work shows a shift from isolated tactic prediction to systems that combine proof synthesis, retrieval, prover feedback, repair, and agentic control. These systems can generate longer proof fragments, use local context, revise failed attempts, and sometimes use informal explanations or proof sketches as guidance. However, proofs in specialized domains such as real-time scheduling often rely on recurring semantic structures, including scheduling assumptions, workload and processor models, invariants, response-time bounds, rewriting conventions, and sequences of lemmas. Existing methods usually treat reusable knowledge as retrieved premises, similar proofs, or short-term proof-state contexts. They do not make domain-specific proof procedures explicit as reusable skills with applicability conditions, required assumptions, expected effects, and adaptation strategies. This leaves a gap between general LLM-based proof generation and domain-aware proof automation for Coq/Rocq libraries. 


